SkipPredict: When to Invest in Predictions for Scheduling

In light of recent work on scheduling with predicted job sizes, we consider the effect of the cost of predictions in queueing systems, removing the assumption in prior research that predictions are external to the system's resources and/or cost-free. In particular, we introduce a novel approach to utilizing predictions, SkipPredict, designed to address their inherent cost. Rather than uniformly applying predictions to all jobs, we propose a tailored approach that categorizes jobs based on their prediction requirements. To achieve this, we employ one-bit "cheap predictions" to classify jobs as either short or long. SkipPredict prioritizes predicted short jobs over long jobs, and for the latter, SkipPredict applies a second round of more detailed "expensive predictions" to approximate Shortest Remaining Processing Time for these jobs. Our analysis takes into account the cost of prediction. We examine the effect of this cost for two distinct models. In the external cost model, predictions are generated by some external method without impacting job service times but incur a cost. In the server time cost model, predictions themselves require server processing time, and are scheduled on the same server as the jobs.

==> motivation.tex <==
\section{Natural experiment: introduction of timers}
\label{sec:natural_exp}


% We examined the mean rating of users over a period of 16 months (between January 2020 and May 2022).
% Figure~\ref{fig:split_corr} shows the correlation between the mean user rating in two consecutive months along with confidence intervals here, via bootstrapping, and users with ratings less than the $20^{th}$ percentile of ratings ($7$ ratings) are excluded.
% The correlation decreases the most in January 2021, which is when the interface was changed.






% 1. Users heterogeneous
% 2. A function of user more than songs
% 3. User interface tunes both of these things.






% \begin{figure}[h]
% \centering
% % \includegraphics[scale=0.5]{graphs/natural_exp/Mean ratio per rating type.png}
% \includegraphics[scale=0.5]{plots_nikhil/naturalexperiment_ratings_distribution.pdf}
% \caption{Mean ratings of each option (dislikes, likes and superlikes) before and after change.}
% \label{fig:mean_rating_before_after}
% \end{figure}



% \begin{figure}[h]
% \centering
% % \includegraphics[scale=0.5]{graphs/natural_exp/Mean user score histogram.png}
% \includegraphics[scale=0.5]{plots_nikhil/naturalexperiment_histogram_user_scores.pdf}
% \caption{Mean user score}
% \label{fig:user_score_hist}
% \end{figure}







% \input{plots_nikhil/naturalexperiment_likeregression.tex}

% \begin{table}[th]
% 	\begin{center}
% 		\begin{tabular}{p{3cm}|p{1cm} |p{1cm}|p{2cm}|p{1cm} |p{1cm} }
% 			\toprule
% 			R-squared & $0.206$ & & & & \\
%             \midrule
%             & coef & t & $P > [t]$ & $0.025$ & $0.975$ \\
% 			\midrule
% 			const & $0.1345$ & $28.316$ & $0.000$ & $0.125$ & $0.144$\\
% 			\midrule
%             mean user factor & $0.2812$& $59.839$& $0.000$& $0.272$& $0.290$ \\
% 			\midrule
%             song factor & $0.3533$& $34.383$& $0.000$& $0.333$& $0.373$ \\
%             \bottomrule
% 		\end{tabular}
% 	\end{center}
% 	\caption{Pre change regression table}
% 	\label{tab:pre_change}
% \end{table}




% \begin{table}[th]
% 	\begin{center}
% 		\begin{tabular}{p{3cm}|p{1cm} |p{1cm}|p{2cm}|p{1cm} |p{1cm} }
% 			\toprule
% 			R-squared & $0.343$ & & & & \\
%             \midrule
%             & coef & t & $P > [t]$ & $0.025$ & $0.975$ \\
% 			\midrule
% 			const & $-0.0615$ & $-10.608$ & $0.000$ & $-0.073$ & $-0.050$\\
% 			\midrule
%             mean user factor & $0.3460$& $63.370$& $0.000$& $0.335$& $0.357$ \\
% 			\midrule
%             song factor & $1.1274$& $112.434$& $0.000$& $1.108$& $1.147$ \\
%             \bottomrule
% 		\end{tabular}
% 	\end{center}
% 	\caption{Post change regression table}
% 	\label{tab:post_change}
% \end{table}





% The reduction indicates that the mean rating per user was influenced by the interface modification, and as a result, it motivated the experiment detailed below.




%Our work focuses on whether we can improve the platform interface design in such a way that it incentivizes users to give real trinary ratings to songs that are aligned with their individual tastes, thus limiting the super-like and pickiness phenomena among users which resulting in quality data.





%TODO: add limitation of the natural experiment
%TODO: Limitations about platform/what is missing from before/after
%Limitation: low traffic in months adjacents to the modifications
% overlap users number was low
%overall users number low
% can't analyze personalied since algorithms changed

%TODO: what will be learned from an actual experiment



==> removed.tex <==
\section{Single-Queue, Server Time Cost}
We consider M/G/1 queueing system with arrival rate $\lambda$. The processing times for each arriving job are independent and drawn based on the cumulative distribution $F(x)$, with an associated density function $f(x)$.
Here, server time cost refers to the time taken by the server to make predictions. Within this framework, predictions are scheduled based on a defined rank function.


A reasonable policy might have predicated short jobs outrank other jobs. Note that to determine whether a job is short or long, it is initially scheduled for a "cheap prediction". Jobs predicted as short are categorized as non-preemptible while in execution, thereby prioritizing their completion before predicting new jobs. However, jobs predicted as long are further scheduled for a detailed "expensive prediction". Thus, cheap predictions outrank expensive predictions and long jobs. Similarly, expensive predictions are prioritized over predicted long jobs.

%{\bf MM:  Should explain here that we make short jobs non-preemptible when running, so predicting new jobs goes behind finishing predicted short jobs -- which makes sense, since even if the jobs were predicted short, they would go to the back of the "short job queue" -- hence the corresponding rank function.}
This hierarchical approach can be viewed as a four-class priority system: Class 1 is designated for short jobs, managed by FCFS within the class. Consequently, short jobs are non-preemptible, thus prioritizing them over predicting new ones. This approach is practical because even if the new jobs are predicted to be short, they are assigned behind the already running short jobs (Following FCFS). Class 2 includes jobs for cheap predictions, also operating under FCFS within their class. Class 3 involves jobs requiring expensive predictions, following the FCFS within the class. Finally, class 4 is reserved for long jobs, according to SPRPT using service time prediction from class 3. 

Following the framework of SOAP policies presented by Scully et al.~\cite{scully2018soap}, we can model the system using descriptor $\mathcal{D} =$ [size, predicted short/long, predicted time] $ = [x, b, r(x)]$ and the following rank function:


\[
rank([x,b, r(x)], a) = 
\begin{cases}
\langle 2, -a \rangle & \text{if $a = 0$ initial rank -- cheap prediction}, \\
\langle 1, -a \rangle & \text{if } b = 1 \text{ and } a > c_1 \text{ (after cheap prediction)}, \\
\langle 3, -a \rangle & \text{if } b = 0 \text{ and } a > c_1 \text{ (after cheap prediction -- expensive prediction)}, \\
\langle 4, r(x) - a \rangle &  \text{ if } b = 0 \text{ and } a > c_1 + c_2 \text{ (after expensive prediction)}.
\end{cases}
\]



\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/rank_function_b_0_rank.png}
    \hspace{0.5cm} % Adds a space between the two figures
    \includegraphics[width=0.45\textwidth]{figs/rank_function_b_1_rank.png}
    \caption{Visual representation of exampled rank function $ rank(d, a) $ for (a) predicted long job ($b = 1$) (b) predicted short job ($b = 0$) (b). Each point combines the first component (class) and the second component (either $-a$ or $ r(x) - a $) into a single value, with the class component represented by color and the second component by position on the y-axis. This visualization demonstrates the relationship between the classes.}

\end{figure}

\colorbox{yellow}{
    \begin{minipage}{\textwidth}
\textbf{simple case:}

For the setting with Poisson arrivals, service times are exponential with a mean of 1.
We consider the exponential prediction model where a prediction of a job with service time $x$ is itself exponentially distributed with mean $x$.
$$f(x) = e^{-x}$$
$$p_T(x) = 1-e^{-\frac{T}{x}}$$
$$g(x,y) = \frac{1}{x}e^{\frac{-y}{x}}$$

$$\int f(x)p_T(x)dx = 1 - \int_{0}^{\infty} e^{-x-\frac{T}{x}}dx = 1- 2\sqrt{T}K_1(2\sqrt{T})$$ Where $K_1$ is a modified Bessel function of the second kind.

$$\int xf(x)p_T(x)dx = \int_{0}^{\infty} xe^{-x} - xe^{-x-\frac{T}{x}}dx = 2- 2T K_2(2\sqrt{T})$$ Where $K_2$ is a modified Bessel function of the second kind (with different parameters).
\end{minipage}
}

\subsection{Mean response time analysis according to SOAP}
In our analysis of the mean response time, we follow the SOAP approach~\cite{scully2018soap}. This analysis uses the tagged-job technique. We focus on a specific job, the 'tagged job', denoted by J, of size $x_J$ and descriptor $d_J$. The mean response time of $J$ is given by the sum of the residence time and the waiting time. To calculate the waiting time, we consider the delays caused by other jobs in the system with $J$. There are two key components: first, determining the delay caused by each ``new'' job (those arriving after J, each denoted by $K$); and second, determining the delay caused by ``old'' jobs (those arriving before J, each denoted by $I$).


Let $q = q$
First, to account for the nonmonotonic rank function, we first compute the worst future rank of $J$, denoted as $rank_{d_J, x_J}^{\text{worst}}$, as follows: 
\[ rank_{d_J, x_J}^{\text{worst}} (a)= \begin{cases} \langle 2, -a \rangle & \text{if $J$ is predicted short} \\ \langle 4, q -a\rangle & \text{if $J$ is predicted long} \end{cases} \] 
When $a_J=0$, the rank function is denoted by $r_{worst}= rank_{d_J, x_J}^{\text{worst}} (0)$.

In the SOAP framework, waiting time is defined as equivalent to the transformed busy period in an M/G/1 system with arrival rate $\lambda$ and job size $X^{\text{new}}[rank_{d_J, x_J}^{\text{worst}} (a)]$ \footnote{$X^{\text{new}}[rank_{d_J, x_J}^{\text{worst}} (a)]$ represents how long a new job that just arrived to the system is served until it completes or surpasses $rank_{d_J, x_J}^{\text{worst}} (a)$}(defined and calculated in section~\ref{sec:soap_x_new}). The initial work of this period represents the delay caused by old jobs.

To deal with the delay due to old jobs, SOAP introduced a transformed system where jobs are categorized based on their rank. \emph{Discarded} old jobs, exceeding the rank threshold $r_{worst}$, are excluded from the transformed system. \emph{Original} old jobs, with a rank at or below $r_{worst}$, are considered as arrivals with rate $\lambda$ and a specific size distribution $X_{0}^{\text{old}}[r_{worst}]$ \footnote{$X_{0}^{\text{old}}[r_{worst}]$ represents how long a job is served while it is considered \emph{original} with respect to the rank $r_{worst}$} (defined and calculated in section~\ref{sec:soap_x_0_old}). \emph{Recycled old jobs}, currently at or below $r_{worst}$ but previously above this threshold, are treated as server vacations of length $X_{i}^{\text{old}}[r_{worst}]$\footnote{$X_{i}^{\text{old}}[r_{worst}]$ represents how long a job is served while it is considered \emph{recycled} for the $i$ time with respect to the rank $r_{worst}$} (defined and calculated in section~\ref{sec:soap_x_i_old}) in the transformed system.

SOAP demonstrates that, because Poisson arrivals see time averages, the stationary delay due to old jobs has the same distribution as queueing time in the transformed M/G/1/FCFS system. This system is characterized by 'sparse' server vacations, where (\emph{original}) jobs arrive at rate $\lambda$ and follow the size distribution $X_{0}^{\text{old}}[r_{worst}]$.

We now proceed to the computation of $X^{\text{new}}[rank_{d_J, x_J}^{\text{worst}} (a)]$, $X_{0}^{\text{old}}[r_{worst}]$ and $X_{i}^{\text{old}}[r_{worst}]$ in our system.


\subsubsection{$X^{\text{new}}[rank_{d_J, x_J}^{\text{worst}} (a)]$ computation:}
\label{sec:soap_x_new}

As mentioned, $X^{\text{new}}[rank_{d_J, x_J}^{\text{worst}} (a)]$ represents how long a new job that just arrived to the system is served until it completes or surpasses $rank_{d_J, x_J}^{\text{worst}} (a)$.
Let's consider a new job $K$ arriving when $J$ is at age $a_J$ (where $a_J \le \min(q, x_J)$). The worst rank of $J$ depends on whether $J$ is predicted to be short or long.
If $J$ is predicted short, then $J$'s worst future rank is its current rank $\langle 2, -a_J \rangle$. 
Given that $K$'s initial rank is $\langle 2, 0 \rangle$, at least equivalent to $J$'s worst future rank, the delay $J$ experiences due to $K$ is:
$$X_{x_K}^{new}[\langle 2, -a_J \rangle] = 0$$.


If $J$ is predicted long, then $J$'s worst future rank is $\langle 4, r(x) - a_J\rangle$. In this case, $J$'s delay due to $K$ also depends on $K$ is predicted to be short or long.
\[X_{x_K}^{new}[\langle 4, q - a_J \rangle]  = 
\begin{cases}
    c_1 + x_K   & \text{$K$ is predicted short } \\
    c_1 + c_2 + x_K \mathds{1}(r(x_K) < q- a_J) & \text{$K$ is predicted long}
\end{cases}
\]


Employing the joint distribution $g(x,y)$, and setting $\mathds{1}(r(x_K) < q - a_J) = \int_{y=0}^{q - a_J} g(x_K,y) dy$, we can derive $J$'s expected delay due to any random new job:




\begin{align*}
\mathbb{E}[X^{new}[\langle 4, q - a_J \rangle]] = & c_1 + \int_{0}^{\infty} p_T(x_K) x_K f(x_K) dx_K \\
& + \int_{0}^{q-a_J} \int_{x_K = 0}^{\infty} (1 - p_T(x_K)) g(x_K,y) \left(c_2 + x_K \right) dx_K dy \\
\end{align*}


\begin{comment}
\begin{align*}
\mathbb{E}[X^{new}[\langle 4, q - a_J \rangle]] = & c_1 + \int_{0}^{\infty} p_T(x_K) x_K f(x_K) dx_K \\
& + \int_{0}^{\infty} (1 - p_T(x_K)) \left(c_2 + x_K \cdot \int_{y=0}^{q - a_J} g(x_K,y) dy \right) f(x_K) dx_K \\
\end{align*}    
\end{comment}



\colorbox{yellow}{
\begin{minipage}{\textwidth}
\textbf{simple case:}
$$\int xf(x)p_T(x)dx = \int_{0}^{\infty} xe^{-x} - xe^{-x-\frac{T}{x}}dx = 1- 2T K_2(2\sqrt{T})$$.
$$\int_{y=0}^{q - a_J} g(x_K,y) dy  = 1- e^{-\frac{1}{x_K} \cdot (q - a_J)}$$

\begin{align*}
\int_{0}^{\infty} (1 - p_T(x_K)) \left(c_2 + x_K \cdot \int_{y=0}^{q - a_J} g(x_K,y) dy \right) f(x_K) dx_K \\ = \int_{0}^{\infty} e^{-x_K -\frac{T}{x_K}} \left(c_2 + x_K - x_K\cdot e^{\frac{-(q - a_J)}{x_K}}\right) dx_K
\\
= c_2 \int_{0}^{\infty} e^{-x_K -\frac{T}{x_K}} dx_K + \int_{0}^{\infty} x_K \cdot e^{-x_K -\frac{T}{x_K}} dx_K - \int_{0}^{\infty} x_K \cdot e^{-x_K -\frac{T+q - a_J}{x_K}} dx_K
\\
= c_2 \cdot 2\sqrt{T}K_1(2\sqrt{T}) + 2T K_2(2\sqrt{T}) - 2(T+q - a_J) K_2(2\sqrt{T+q - a_J})
\end{align*}


\begin{align*}
    \mathbb{E}[X^{new}[\langle 4, q - a_J \rangle]] = c_1 + c_2 \cdot 2\sqrt{T}K_1(2\sqrt{T}) - 2(T+q - a_J) K_2(2\sqrt{T+q - a_J})
\end{align*}
\end{minipage}
}


\subsubsection{$X_{0}^{\text{old}}[r_{worst}]$ computation:}
\label{sec:soap_x_0_old}

$X_{0}^{\text{old}}[r_{worst}]$ represents how long a job is served while its age is in its $0$-old $r_{worst}$-interval. This interval, as defined in SOAP (Definition 4.5), refers to the interval of ages during which a job is original with respect to rank $r_{worst}$.

We start by computing the relevant intervals according to our rank function. In our case, all jobs start with $\langle 2, 0 \rangle$ rank. Suppose that $J$ witnesses an old job $I$ of initial size $x_I$. The duration for which $I$ remains \emph{original} depends on whether its prediction is short or long.

if $J$ is predicted short, $r_{worst} = \langle 2, 0 \rangle$, if $I$ is also predicted short, its $0$-old $r_{worst}$-interval spans from $0$ to $\infty$, meaning that $I$ remains original until completion. Here, $X_{0}^{\text{old}}[r_{worst}] = c_1 + x_I$. Alternatively, if $I$ is predicted long, its $0$-old $r_{worst}$-interval is $[0, c_1]$, since after completing the cheap prediction phase (lasting $c_1$), its rank shifts to $\langle 3, 0 \rangle$. In this instance, $X_{0}^{\text{old}}[r_{worst}] = c_1$. Therefore, we have:

\[
X_{0, x_I}^{\text{old}}[\langle 2, 0 \rangle] = 
\begin{cases}
    c_1 + x_I   & \text{if $I$ is predicted short} \\
    c_1 & \text{if $I$ is predicted long}
\end{cases}
\]



\begin{align*}
\mathbb{E}[X_0^{\text{old}}[\langle 2, 0 \rangle]] =  c_1 + \int_{0}^{\infty} p_T(x_I) x_I f(x_I) dx_I
\end{align*}




\colorbox{yellow}{
\begin{minipage}{\textwidth}
\textbf{simple case:}
$$\mathbb{E}[X_0^{\text{old}}[\langle 2, 0 \rangle]] = c_1 + 1- 2T K_2(2\sqrt{T})$$
\end{minipage}
}



\begin{align*}
\mathbb{E}[X_0^{old}[\langle 2, 0 \rangle]^2]] =  \int_{0}^{\infty} p_T(x_I) (c_1 + x_I)^2 f(x_I) dx_I + \int_{0}^{\infty} (1-p_T(x_I)) \cdot c_1^2 \cdot f(x_I) dx_I \\
= c_1^2 + 2c_1 \int_{0}^{\infty} p_T(x_I) x_I f(x_I) dx_I + \int_{0}^{\infty} p_T(x_I) x_I^2 f(x_I) dx_I
\end{align*}

\colorbox{yellow}{
\begin{minipage}{\textwidth}
\textbf{simple case:}
\begin{align*}
\mathbb{E}[X_0^{old}[\langle 2, 0 \rangle]^2]] = c_1^2 + 2c_1 \cdot (1- 2T K_2(2\sqrt{T})) + \int_{0}^{\infty}(1-e^{\frac{-T}{x_I}}) e^{-x_I} x_I^2 dx_I \\
= c_1^2 + 2c_1 \cdot (1- 2T K_2(2\sqrt{T})) + \int_{0}^{\infty} x_I^2 e^{-x_I} dx_I - \int_{0}^{\infty} x_I^2 e^{-x_I-\frac{T}{x_I}} dx_I \\
= c_1^2 + 2c_1 \cdot (1- 2T K_2(2\sqrt{T})) + 2 - 2T^{1.5} K_3(2\sqrt{T}) \rana{recheck $K_3$..}
\end{align*}

\end{minipage}
}



If $J$ is predicted long, $r_{worst} = \langle 4, q \rangle$. In this scenario, regardless of $I$'s prediction, the $0$-old $r_{worst}$-interval for $I$ spans from $0$ to $\infty$. This implies that $X_{0, x_I}^{\text{old}}[\langle 4, q \rangle]$ represents the entire service duration of $I$. Thus:

\[
X_{0, x_I}^{\text{old}}[\langle 4, q \rangle] = 
\begin{cases}
    c_1 + x_I   & \text{if $I$ is predicted short} \\
    c_1 + c_2 + x_I \cdot \mathds{1}(r(x_I) \le q) & \text{if $I$ is predicted long}
\end{cases}
\]





\begin{align*}
\mathbb{E}[X_{0}^{\text{old}}[\langle 4, q \rangle]] = & c_1 + \int_{0}^{\infty} p_T(x_I) x_I f(x_I) dx_I \\
& + \int_{y = 0}^{q} \int_{x_I = 0}^{\infty} (1 - p_T(x_I)) g(x_I,y) \left(c_2 + x_I  \right)  dx_I dy \\
\end{align*}


\colorbox{yellow}{
\begin{minipage}{\textwidth}
\textbf{simple case:}
\begin{align*}
    \mathbb{E}[X_{0}^{\text{old}}[\langle 4, q \rangle]]  = c_1 + c_2 \cdot 2\sqrt{T}K_1(2\sqrt{T}) - 2(T+q) K_2(2\sqrt{T+q})
\end{align*}
\end{minipage}
}

\begin{align*}
\mathbb{E}[(X_{0}^{\text{old}}[\langle 4, q \rangle])^2]] = &  \int_{0}^{\infty} p_T(x_I) (c_1 + x_I)^2 f(x_I) dx_I + \\
& \int_{y = 0}^{q} \int_{x_I = 0}^{\infty} (1-p_T(x_I)) \cdot g(x_I, y) \left(c_1 + c_2 + x_I\right)^2  dx_I dy
\end{align*}





\colorbox{yellow}{
\begin{minipage}{\textwidth}
\textbf{simple case:}

\begin{align*}
    \mathbb{E}[(X_{0}^{\text{old}}[\langle 4, q \rangle])^2]] =  c_1^2 \left(1- 2\sqrt{T}K_1(2\sqrt{T})\right) + 2c_1 \cdot (1- 2T K_2(2\sqrt{T})) + 2 - 2T^{1.5} K_3(2\sqrt{T})  \\ + \int_{0}^{\infty} e^{-x_K -\frac{T}{x_K}} \left(c_1 + c_2 + x_K(1-e^{\frac{-q}{x_K}})\right)^2 dx_K
\end{align*}


\begin{equation*}
\begin{aligned}
\left(c_1 + c_2 + x_K\left(1-e^{-\frac{q}{x_K}}\right)\right)^2 &= (c_1 + c_2)^2 + \left(x_K\left(1-e^{-\frac{q}{x_K}}\right)\right)^2 \\
&\quad+ 2(c_1 + c_2)x_K\left(1-e^{-\frac{q}{x_K}}\right) \\
&= (c_1 + c_2)^2 + x_K^2\left(1 - 2e^{-\frac{q}{x_K}} + e^{-\frac{2q}{x_K}}\right) \\
&\quad+ 2(c_1 + c_2)x_K\left(1-e^{-\frac{q}{x_K}}\right).
\end{aligned}
\end{equation*}



\begin{equation*}
\begin{aligned}
 \int_{0}^{\infty} e^{-x_K -\frac{T}{x_K}} \left(c_1 + c_2 + x_K(1-e^{\frac{-q}{x_K}})\right)^2 dx_K = (c_1 + c_2)^2 2\sqrt{T}K_1(2\sqrt{T}) + 4(c_1+c_2)T K_2(2\sqrt{T}) \\
 - 4(c_1+c_2)(T+q)K_2(2\sqrt{T+q}) +  2T^{1.5} K_3(2\sqrt{T}) \\
 -4(T+q)^{1.5} K_3(2\sqrt{T+q}) + 2(T+2q)^{1.5} K_3(2\sqrt{T+2q})
\end{aligned}
\end{equation*}


\begin{align*}
    \mathbb{E}[(X_{0}^{\text{old}}[\langle 4, q \rangle])^2]] =  (c_1^2 + 2c_1 + 2) + (c_2(2c_1+c_2))\left(2\sqrt{T}K_1(2\sqrt{T})\right) + 4c_2 T K_2(2\sqrt{T}) \\ - 4(c_1+c_2)(T+q)K_2(2\sqrt{T+q})\\
 -4(T+q)^{1.5} K_3(2\sqrt{T+q}) + 2(T+2q)^{1.5} K_3(2\sqrt{T+2q})
\end{align*}


\end{minipage}
}



\subsubsection{$X_{i}^{\text{old}}[r_{worst}]$ computation:}
\label{sec:soap_x_i_old}

For $i \ge 1$, $X_{i}^{\text{old}}[r_{worst}]$ represents how long a job is served while it is considered \emph{recycled} for the $i$ time with respect to the rank $r_{worst}$.

If $J$ is predicted short, $r_{worst} = \langle 2, 0 \rangle$, there are no instances of recycled jobs. This is because either $I$ completes its service (if predicted short) or it is discarded completely (if predicted long), and thus never gets a rank lower than $\langle 2, 0 \rangle$. As a result, for $i \ge 1$, $$X_{i, x_I}^{\text{old}}[\langle 2, 0 \rangle] = 0$$.

If $J$ is predicted long, job $I$ may be recycled. This occurs when $I$ is predicted as long and with an expensive prediction $r(x_I) > q$. $I$ is initially considered as \emph{original} and is served during the cheap and expensive prediction phases, then discarded. At age $a_I = r(x_I) - q$, $I$ is recycled and served till completion, which will be $x_I - a_I = x_I - (r(x_I) - q)$.

Thus, we have:
\[
X_{1, x_I}^{\text{old}}[\langle 4, q \rangle] =
\begin{cases}
    0   & \text{if $I$ is predicted short} \\
    x_I - (r(x_I) - q) & \text{if $I$ is predicted long}
\end{cases}
\]
For $i \ge 2$, $$X_{i, x_I}^{\text{old}}[\langle 2, q \rangle] = 0$$

let $t = r(x_I)$

\begin{align*}
\mathbb{E}[X_{1}^{\text{old}}[\langle 4, q \rangle]^2] = \int_{t = q}^{\infty} \int_{x_I = t-q}^{\infty} (1-p_T(x_I)) \cdot g(x_I, t)\cdot(x_I - (t - q))^2 \cdot dx_I dt
\end{align*}

\colorbox{yellow}{
\begin{minipage}{\textwidth}
\textbf{simple case:}
\rana{EDIT}
$r(x_I) = \int_{0}^{\infty} y(\frac{1}{x_I} e^{\frac{-y}{x_I}}) dy = x_I $
\begin{align*}
    \mathbb{E}[X_{1}^{\text{old}}[\langle 4, q \rangle]^2] = \int_{0}^{\infty} e^{-x_I-\frac{T}{x_I}} \cdot (x_I - x_I + q)^2 dx_I = q^2 \cdot (1- 2\sqrt{T}K_1(2\sqrt{T}))
\end{align*}

\end{minipage}
}


\subsubsection{Applying SOAP}

Let
\begin{itemize}
    \item $X_{PL}$ and $X_{PS}$ be the respective size distribution of predicted long jobs and predicted short jobs.
\end{itemize}

Applying Theorem 5.5 of SOAP~\cite{scully2018soap} yields the following mean response times:

\begin{align*}
\mathbb{E}[T_{x_J\text{- predicted short}}] = & \frac{\lambda \cdot \mathbb{E}[X_0^{old}[\langle 2, 0 \rangle]^2]}{2(1-\lambda \mathbb{E}[X_0^{old}[\langle 2, 0 \rangle]]) (1-\lambda\mathbb{E}[X^{new}[\langle 2, 0 \rangle]])} + \int_{0}^{x_J} \frac{1}{1-\lambda\mathbb{E}[X^{new}[\langle 2, -a \rangle]]} da \\
& = \frac{\lambda \cdot \mathbb{E}[X_0^{old}[\langle 2, 0 \rangle]^2]}{2(1-\lambda \mathbb{E}[X_0^{old}[\langle 2, 0 \rangle]])} + \mathbb{E}[X_{PL}] = \frac{\lambda \cdot \mathbb{E}[X_0^{old}[\langle 2, 0 \rangle]^2]}{2(1-\rho_{0_{PS}}^{old})} + \mathbb{E}[X_{PL}]
\end{align*}

where $\rho_{0_{PS}}^{old} = \lambda \mathbb{E}[(X_0^{old}[\langle 2, 0 \rangle])$


\colorbox{yellow}{
\begin{minipage}{\textwidth}
\textbf{simple case:}

\mathbb{E}[T_{x_J\text{- predicted short}}] = \frac{ \lambda \cdot ( c_1^2 + 2c_1 \cdot (1- 2T K_2(2\sqrt{T})) + 2 - 2T^{1.5} K_3(2\sqrt{T}))}{2(1-\lambda(c_1 + 1- 2T K_2(2\sqrt{T}))} + \mathbb{E}[X_{PL}]
\end{minipage}
}

\colorbox{orange}{
\begin{minipage}{\textwidth}
\textbf{$\mathbb{E}[T_{x_J\text{- predicted short}}]$ analysis without SOAP theorem:}
If $J$ is predicted short, new arriving jobs do not preempt $J$. This is because if $J$ is undergoing its cheap prediction phase, it will, by FCFS during this phase, be queued ahead of the new job. Alternatively, if $J$ is already at the highest class (i.e., lowest rank), it will not be subject to preemption. As a result, the mean response time for $J$ is the sum of its waiting time and the size; \mathbb{E}[T_J] = \mathbb{E}[T_Q] + \mathbb{E}[X_J]$.

In addition, in this context, there are no recycled jobs, as discussed in Section~\ref{sec:soap_x_i_old}. This implies that the only delay $J$ experiences is from old jobs, equating to the waiting time in an FCFS system without server vacations, where the job size distribution in this scenario corresponds to $X_0^{\text{old}}[\langle 2, 0 \rangle]$.

To calculate the waiting time, we apply Equation 23.15 from~\cite{harchol2013performance}: $\mathbb{E}[T_Q] = \frac{\lambda \mathbb{E}[S^2]}{2(1-\rho)}$. By setting the job size distribution to $X_0^{\text{old}}[\langle 2, 0 \rangle]$, we can derive the desired result.
\end{minipage}
}






\begin{align*}
\mathbb{E}[T_{x_J\text{- predicted long with size $x_J$}}] =  & \frac{\lambda \cdot (\mathbb{E}[X_0^{old}[\langle 4, q \rangle]^2] + \mathbb{E}[X_1^{old}[\langle 4, q \rangle]^2])}{2(1-\lambda \mathbb{E}[X_0^{old}[\langle 4, q \rangle]) (1-\lambda\mathbb{E}[X^{new}[\langle 4, q \rangle])} \\
& +\int_{0}^{x_J} \frac{1}{1-\lambda\mathbb{E}[X^{new}[\langle 4, q - a \rangle]]} da
\end{align*}


\colorbox{orange}{
\begin{minipage}{\textwidth}
\textbf{$\mathbb{E}[T_{x_J\text{- predicted long with size $x_J$}}]$ analysis without SOAP theorem:}
If $J$ is predicted long, the delay from newly arriving jobs is incorporated into $J$'s waiting time. We approach the analysis of $J$'s waiting time by considering the length of the busy period for new arrivals, characterized by a job size distribution $X^{\text{new}}[\langle 4, q \rangle]$. This period begins with an initial workload $W$, representing an old jobs delay.

As shown in Equation 27.7 from~\cite{harchol2013performance}, the mean length of this busy period is given by $\mathbb{E}[B_W] = \frac{\mathbb{E}[W]}{1-\rho_{\text{new}}} = \frac{\mathbb{E}[W]}{1-\lambda \mathbb{E}[X^{\text{new}}[\langle 4, q \rangle]]}$. This workload $W$ is equivalent to the waiting time in an FCFS system with server vacations, where jobs arrive at rate $\lambda$ and have a size distribution $X_0^{\text{old}}[\langle 4, q \rangle]$.

In our model, we consider a single type of vacation, the length of which is determined by the distribution $X_1^{\text{old}}[\langle 4, q \rangle]$ (see section~\ref{sec:soap_x_i_old}). Following Section 27.2 in~\cite{harchol2013performance}, the Laplace-Stieltjes transform of the waiting time in an M/G/1 queue with vacations of length $V$ is $\tilde{T}^{M/G/1/\text{Vac}}(s) = \tilde{T}^{M/G/1}(s) \cdot \tilde{V_e}(s)$, where $\tilde{V_e}(s)$ is the excess of $V$. Therefore, the expected total time in an M/G/1 queue with vacations is $E[T]^{M/G/1/\text{Vac}} = E[T]^{M/G/1} + E[V_e]$. --\rana{recheck.}

To compute $E[T]^{M/G/1/\text{Vac}}$, we use Equation 23.15 from~\cite{harchol2013performance}: $\mathbb{E}[T_Q] = \frac{\lambda \mathbb{E}[S^2]}{2(1-\rho)}$, applying the job size distribution $X_0^{\text{old}}[\langle 4, q \rangle]$ for this calculation.

For the calculation of $V_e$, we refer to Equation 23.15 from~\cite{harchol2013performance}
....
\end{minipage}
}


\colorbox{yellow}{
\begin{minipage}{\textwidth}
\textbf{simple case:}

\mathbb{E}[T_{x_J\text{- predicted long with size $x_J$}}]  = 






\end{minipage}
}




\begin{comment}
Cheap predictions is uniform prediction model: predictions are uniformly distributed between 0 and a maximum value $M$ ($T \le M$). The formula for $ p_T(x) $ is:
$p_T(x) = \frac{T}{M} $
Expensive prediction is a linear prediction model: The predicted size $ y $ is a fixed proportion $ k $ of the actual size $ x $. The joint density function $ g(x, y) $ is:
\begin{equation}
g(x, y) = e^{-x} \cdot \delta(y - kx)
\end{equation}
In this setting, ....
\end{comment}

\subsection{Total Expected Cost}
We model the total expected cost as $$(1-z) \cdot \mathbb{E}[T_{x_J\text{- predicted long}}] + z \cdot \mathbb{E}[T_{x_J\text{- predicted long}}] $$ 


%calc second moment of x_0_old, x_1_old, 
% calc soap equations
%derive equations without SOAP..
% simple example to verify


%===============


\subsection{Baselines}

As baselines, we compare our model to two single-queue models with service time to compute the predictions. These models are preemptive, running either expensive predictions for all jobs with SPRPT or cheap predictions for all jobs with FCFS.


\section{Model 1 and 2 comparison}



\begin{table}[h]
\centering
\caption{Models Comparison in terms of mean response time}
\label{tab:dataset_comparison}
\begin{tabular}{@{}lcc@{}}
\toprule
Job Predicted & Model 1 & Model 2\\ \midrule
Short & $\frac{\lambda \left(2- 2T^{1.5} K_3(2\sqrt{T}) \right)}{2\left(1-  \lambda \left(1- 2T K_2(2\sqrt{T} \right)\right)} + \mathbb{E}[S_1']$ & $ \frac{ \lambda \cdot \left( c_1^2 + 2c_1 \cdot (1- 2T K_2(2\sqrt{T})) + 2 - 2T^{1.5} K_3(2\sqrt{T})\right)}{2\left(1-\lambda(c_1 + 1- 2T K_2(2\sqrt{T})\right)} + \mathbb{E}[S_1']$ \\
Long & [TODO] & [TODO] \\
\bottomrule
\end{tabular}
\end{table}



\begin{comment}
    
\subsection{REMOVE}



Again, if $J$ is predicted short, then $I$ delayed $J$ only if $I$ is predicted short, otherwise $J$ prioritized $I$. Also, $I$ is never recycled since it completes (when predicted as short) before $J$:





\[X_{0, x_I}^{old}[\langle 2, 0 \rangle] = 
\begin{cases}
    c_1 + x_I   & \text{$I$ is predicted short} \\
    c_1 & \text{$I$ is predicted long}.
\end{cases}
\]

\[X_{1,x_I}^{old}[\langle 2, 0 \rangle] =  0\]




\[X_{0, x_I}^{old}[\langle 2, 0 \rangle] = 
\begin{cases}
    c_1 + x_I   & \text{$I$ is predicted short and I's rank $\langle 2, 0 \rangle$} \\
    x_I & \text{$I$ is predicted short and I's rank $\langle 1, 0 \rangle$}.
\end{cases}
\]

\[X_{1,x_I}^{old}[\langle 2, 0 \rangle] =  0\]

Thus, in this case the delay due to any original old job is:
\begin{align*}
\mathbb{E}[X_{0}^{old}[\langle 2, 0 \rangle]] = & \int_{0}^{\infty} p_T(x_I) (c_1 + x_I) f(x_I) dx_I \cdot \mathds{1}_{\text{Age is 0 / rank <2,0> } } \\
& + \int_{0}^{\infty} p_T(x_I) x_I f(x_I) dx_I \cdot \mathds{1}_{\text{Age is } c_1/ rank <1,0>}
\end{align*}


\rana{how we can calc these $\mathds{1}_{\text{Age is */rank<*,*>}}$?, should we consider steady-state probabilities of other jobs in the system because it doesnt make sense to me to calc the probability of rank function?}

If $J$ is predicted long, it will be delayed by $I$ in any case, where the delay length depends on $I$'s rank.


\[X_{0, x_I}^{old}[\langle 4, q \rangle] = 
\begin{cases}
    c_1 + x_I   & \text{$I$ is predicted short and I's rank $\langle 2, 0 \rangle$} \\
    c_1 + c_2 + x_I \mathds{1}(r(x_I) \le q) & \text{$I$ is predicted long and I's rank $\langle 2, 0 \rangle$} \\
    x_I & \text{$I$ is predicted short and I's rank $\langle 1, 0 \rangle$} \\
    c_2 + x_I \mathds{1}(r(x_I) \le q)   & \text{$I$ is predicted long and I's rank $\langle 3, 0 \rangle$} \\
    x_I \mathds{1}(r(x_I) \le q)   & \text{$I$ is predicted long and I's rank $\langle 4, 0 \rangle$}
\end{cases}
\]


In addition, in this case ($J$ is predicted as long), there may be instances where $I$ gets recycled. This situation can occur if $I$, initially predicted as long, was preempted by other jobs and later -- when $q \ge r(x_I) - a_I$ -- becomes visible again. In such cases, $I$ will be recycled at an age $a_I = r(x_I) - q$ and delay $J$ by $x_I - a_I = x_I -r(x_I) + q$.


\[X_{1, x_I}^{old}[\langle 4, q \rangle]] =
\begin{cases}
    0   & \text{$I$ is predicted short} \\
    x_I -r(x_I) + q & \text{$I$ is predicted long}
\end{cases}
\]




Similarly, the delay caused by any original old job is:




\begin{align*}
\mathbb{E}[X_{0}^{old}[\langle 4, q \rangle]] = & \int_{0}^{\infty} p_T(x_I) (c_1 + x_I) f(x_I) dx_I \cdot \mathds{1}_{\text{Age is 0 / rank <2,0>}} \\
& + \int_{0}^{\infty} (1 - p_T(x_I)) (c_1 + c_2 + x_I \int_{y=0}^{q} g(x_K,y) dy) f(x_I) dx_I \cdot \mathds{1}_{\text{Age is 0 / rank <2,0>}} \\
& + \int_{0}^{\infty} x_I f(x_I) dx_I \cdot \mathds{1}_{\text{Age is } c_1 / rank <1,0>} \\
& + \int_{0}^{\infty} \left(c_2 + x_I \int_{y=0}^{q} g(x_K,y) dy \right) f(x_I) dx_I \cdot \mathds{1}_{\text{Age is } c_1 / rank <3,0>} \\
& + \int_{0}^{\infty} \left(x_I \int_{y=0}^{q} g(x_K,y)dy \right) \cdot f(x_I) dx_I \cdot \mathds{1}_{\text{Age is } c_1 + c_2 / rank <4,0>}
\end{align*}


\rana{??
\begin{align*}
\mathds{1}_{\text{Age is 0 / rank <2,0>}} = \text{The probability that $x_I$ has not yet received any service} == \text{server is busy and there are jobs with ranks <2,0>??}
\end{align*}
\begin{align*}
\mathds{1}_{\text{Age is $c_1$}} = \text{$x_I$ preempted at age $c_1$} == \text{}
\end{align*}}



\end{comment}



\begin{comment}




\[\mathbb{E}[(X_0^{old}[\langle 2, 0 \rangle]] = c_1 + x_I \cdot p_T(x_I)\]


\[\mathbb{E}[X_{0, x_I}^{old}[\langle 4, q \rangle]] = c1 + (1-p_T(x_I)) \cdot (c_2 + \mathds{1}(r(x_I) \le q) \cdot x_I) + p_T(x_I) \cdot x_I\]

\[\mathds{1}(r(x_I) \le q) = \int_{y=0}^{q} g(x_K,y) dy\]

\[\mathbb{E}[(X_1^{old}[\langle 4, q \rangle]] = x_J \cdot (1-p_T(x_I))\]

Applying Theorem 5.5 of SOAP~\cite{scully2018soap} yields the following mean response times:

\[
\mathbb{E}[T_{x_J\text{- predicted short}}] = \frac{\lambda \cdot (\mathbb{E}[(X_0^{old}[\langle 2, 0 \rangle])^2 + \mathbb{E}[(X_1^{old}[\langle 2, 0 \rangle])^2])}{2(1-\lambda \mathbb{E}[(X_0^{old}[\langle 2, 0 \rangle]) (1-\lambda\mathbb{E}[X^{new}[\langle 2, 0 \rangle]])} + \int_{0}^{x_J} \frac{1}{1-\lambda\mathbb{E}[X^{new}[\langle 2, 0 \rangle]]} da = \frac{\lambda\cdot \left(c_1 + x_I \cdot p_T(x_I)\right)^2}{2(1-\lambda(c_1 + x_I \cdot p_T(x_I))} + x_J
\]


\[
\mathbb{E}[T_{x_J\text{- predicted long}}] = \frac{\lambda \cdot (\mathbb{E}[(X_0^{old}[\langle 4, q \rangle])^2 + \mathbb{E}[(X_1^{old}[\langle 4, q \rangle])^2])}{2(1-\lambda \mathbb{E}[(X_0^{old}[\langle 4, q \rangle]) (1-\lambda\mathbb{E}[X^{new}[\langle 4, q \rangle])} + \int_{0}^{x_J} \frac{1}{1-\lambda\mathbb{E}[X^{new}[\langle 4, r(x_J - a) \rangle]]} da
\]


\begin{align*}
\frac{\lambda \left( x_J^2(p_T(x_I) - 1)^2 + \left( p_T(x_I)(c_1 + x_I) - (p_T(x_I) - 1)(c_1 + c_2 + \mathds{1}(r(x_I) \le q) x_I) \right)^2 \right)}{2 \left( \lambda \left( \lambda \left( p_T(x_K)(c_1 + x_K) - (p_T(x_K) - 1)(c_1 + c_2 + \mathds{1}(r(x_K) < q) x_K) \right) - 1 \right) \left( p_T(x_I)(c_1 + x_I) - (p_T(x_I) - 1)(c_1 + c_2 + \mathds{1}(r(x_I) \le q) x_I) \right) + 1 \right)} \\
+ \int_{0}^{x_J} \frac{1}{1-\lambda\mathbb{E}[X^{new}[\langle 4, r(x_J - a) \rangle]]} da
\end{align*}




\begin{itemize}
    \item $I$ is predicted short, either way if $J$ is predicted short (due to FCFS tiebreaking) or long
    \[
    X_{0, x_I}^{old}[\langle 2, 0 \rangle] =  c_1 + x_I\]
    \[X_{0, x_I}^{old}[\langle 4, q \rangle] =  c_1 + x_I
    \]
    $I$ is never recycled, so $X_{i}^{old}[\langle 2, 0 \rangle] = 0$

    
    
    \item $I$ is predicted long, $J$ is predicted short:
    \[
    X_{0, x_I}^{old}[\langle 2, 0 \rangle] =  c_1
    \]


    \item $I$ is predicted long, $J$ is predicted long:
    \[
    X_{0, x_I}^{old}[\langle 4, q \rangle] =  c_1 + c_2 + x_I \mathds{1}(r(x_I) \le q)
    \]

\end{itemize}








%See analysis page 24, split E[T_{j predcited short}] and E[T_{j predcited long}]
%when j predicted short, the rank function is monotonic, making it easier to analyze
%consider ratio c2 and c1
%change params in code


\begin{itemize}
    \item $J$ is predicted short \rana{becuase we are looking at the moment $J$ arrives}
    \[
    X_0^{old}[\langle 2, 0 \rangle] =  c_1 \cdot \text{\#jobs with descriptor $\langle 2, -a \rangle$} + E[S_{\text{short}}] \cdot \text{\#predicted short jobs -- rank $\langle 1, * \rangle$}
    \]

    \item  $J$ is predicted long
    \begin{align*}
    X_0^{old}[\langle 4, q \rangle] =\ & c_1 \cdot \text{\#jobs with descriptor $\langle 2, -a \rangle$} \\
    & + E[S_{\text{short}}] \cdot \text{\#jobs with rank $\langle 1, -a \rangle$} \\
    & + c_2 \cdot \text{\#jobs with rank $\langle 3, -a \rangle$} \\
    & + \text{jobs with class 4 remaining time less than $x_I - a_J$}
    \end{align*}

\end{itemize}



%=============================

(2) $J$ is delayed by new jobs (considered in case 1) and by old jobs (considered in case 2).

\textit{Case 1 - New jobs delaying $J$:} We compute the delay caused by new jobs, denoted as $X^{new}[r^{worst}]$.

Suppose that a new job $K$ arrives when $J$ has age $a_J$.
\begin{itemize}
    \item $J$ is predicted short ($J$ goes from $\langle 2, -a \rangle$ to $\langle 1, -a \rangle$): $J$'s worst future rank is its current rank $\langle 2, -a_J \rangle$, $K$'s initial rank is $\langle 2, 0 \rangle$, which is at least $J$'s worst future rank. This means $J$'s delay due to $K$ is $$X^{new}[\langle 2, 0 \rangle] = 0$$.

    \item  $J$ is predicted long ($J$ goes from $\langle 2, -a \rangle$,  $\langle 3, -a \rangle$, to $\langle 4, r(x) -a \rangle$): $J$'s worst future rank is $\langle 4, r(x) \rangle$

    \[X_{x_K}^{new}[\langle 4, q - a_J \rangle]  = 
    \begin{cases}
        c_1 + x_K   & \text{$K$ is predicted short } \\
        c_1 + c_2 + x_K \mathds{1}(r(x_K) < q- a_J) & \text{$K$ is predicted long}.
    \end{cases}
    \]
\end{itemize}



\[\mathbb{E}[X^{new}[\langle 4, q \rangle]] = c_1 + p_T(x_K) \cdot x_K + (1 - p_T(x_K)) \cdot (c_2 + \mathds{1}(r(x_K) < q) \cdot x_K)
\]
\[\mathds{1}(r(x_K) < q) = \int_{y=0}^{q - 1} g(x_K,y) dy\]


\[\mathbb{E}[X^{new}[\langle 4, r(x_J - a) \rangle]] = c_1 + p_T(x_K) \cdot x_K + (1 - p_T(x_K)) \cdot (c_2 + \mathds{1}(r(x_K) < q - a) \cdot x_K)
\]
\[\mathds{1}(r(x_K) < q - a_J) = \int_{y=0}^{q - a_J - 1} g(x_K,y) dy\]
\[a_J \le min(q, x_J)\]



We need to know J's delay due to a random new job, meaning one with size drawn from the size distribution $X$, we replace $x_K$ with $X$. \rana{TODO: or we do integral over $x_K$ sizes?}



\begin{itemize}
    \item When $ I $'s Age is 0 / rank <2,0> (rank $ \langle 2, 0 \rangle $):
    \begin{itemize}
        \item Predicted short: $ P_{\text{short}, 2,0} = p_T(x_I) $, Value: $ c_1 + x_I $
        \item Predicted long: $ P_{\text{long}, 2,0} = 1 - p_T(x_I) $, Value: $ c_1 + c_2 + x_I \mathds{1}(r(x_I) \le q) $
    \end{itemize}
    
    \item When $ I $'s age is $ c_1 $ (rank $ \langle 1, 0 \rangle $, $ \langle 3, 0 \rangle $):
    \begin{itemize}
        \item Predicted short (rank $ \langle 1, 0 \rangle $): Value: $ x_I $
        \item Predicted long (rank $ \langle 3, 0 \rangle $): Value: $ c_2 + x_I \mathds{1}(r(x_I) \le q) $
    \end{itemize}

    \item When $ I $'s age is $ c_1 + c_2 $ (rank $ \langle 4, 0 \rangle $):
    \begin{itemize}
        \item Predicted long: Value: $ x_I \mathds{1}(r(x_I) \le q) $
    \end{itemize}
\end{itemize}





\end{comment}



$$\lambda'_1 = \lambda \int_{0}^{\infty} f(x) p_T(x) \, dx = \lambda \cdot (1-z); \lambda'_2 = \lambda \int_{0}^{\infty} f(x) (1-p_T(x)) \, dx = \lambda \cdot z$$




\subsection{MODEL 1: Mean response time for predicted long job:}
\rana{FOLLOW SOAP - WRITE FOR GENERAL PREDICTED + SRPT then for model 2}

To calculate the mean response time of $subsystem_2$, we follow the framework of Mitzenmacher~\cite{mitzenmacher2019scheduling} that extends the SRPT policy to predictions using the same notation of $g(x,y)$ but with slightly different calculations, as only long jobs are considered for this subsystem. Additionally, we consider the slowdown caused by preemption due to short jobs.


Let $f_p(y) = \int_{x=0}^{\infty} g(x,y) dx$; $\rho'_y = \lambda \int_{t=0}^{y} \int_{x=0}^{\infty} g(x,t) x dx dt$.
The following is known (see Section (4c) of~\cite{mitzenmacher2019scheduling}:
\begin{flalign}
\mathbb{E}[T]^{SPRPT} = \int_{y=0}^{\infty} f_p(y)\mathbb{E}[W(y) + R(y)]dy \label{eq_SPRPT}
\end{flalign}

Where:
\begin{flalign*}
& \mathbb{E}[W(q)] = b(q) \left(\frac{a_2(q)}{2a_1(q)(1-\rho'_q)} + \lambda F_p(q)\frac{\mathbb{E}[X(q)^2]}{2(1-\rho'_q)^2}\right) \\
& \mathbb{E}[R(y)] = \int_{x=0}^{\infty} \frac{g(x,y)}{f_p(y)} \int_{t=0}^{x} \frac{dt}{1- \rho_{{(y-t)^{+}}}} dx\\
& F_p(q) = \int_{x=0}^{q} f_p(x) dx \\
& \mathbb{E}[X(q)^2] = \frac{1}{F_p(q)} \int_{t=0}^{q} \int_{x=0}^{\infty} g(x,t) x^2 dx dt \\
& b(q) = \rho'_q + \lambda\int_{t=1}^{\infty} g(x,t)(x-(t-q))^{+} dx dt \\
& a_1(q) = (1-b(q))\int_{t=0}^{q} \int_{x=0}^{\infty} g(x,t)x dx dt + \int_{t=q}^{\infty} \int_{x=t-q}^{\infty} g(x,t)(x-(t-q)) dx dt \\
& a_2(q) = (1-b(q))\int_{t=0}^{q} \int_{x=0}^{\infty} g(x,t)x^2 dx dt + \int_{t=q}^{\infty} \int_{x=t-q}^{\infty} g(x,t)(x-(t-q))^2 dx dt
\end{flalign*}



%%%%%%%%%%%%%

Considering only predicted long jobs, we let:


$$\rho'_{2_y}= \lambda'_2 \int_{t=0}^{y} \int_{x=0}^{\infty} g(x,t)x dx dt = z \lambda \int_{t=0}^{y} \int_{x=0}^{\infty} g(x,t)x dx dt = z \rho'_y $$

$\rho'_{2_y}$ is the load associated with predicted jobs of predicted service time up to $y$.
The expression from~\eqref{eq_SPRPT} make use of $\rho'_y$ and $\lambda$. For our subsystem we use $\rho'_{2_y}$ and $\lambda'_2$ instead.
Also, since any predicted short job will preempt the job, we multiply by $\frac{1}{1-\rho'_1}$:


\begin{flalign}
\mathbb{E}[T]^{SPRPT_{subsystem_2}} = \frac{1}{1-\rho'_1} \int_{y=0}^{\infty} f_p(y)\mathbb{E}[W'(y) + R'(y)] \, dy
\end{flalign}

Where:
\begin{flalign*}
& b'(q) = \rho'_{2_q} + \lambda'_2 \int_{t=1}^{\infty} g(x,t)(x-(t-q))^{+} dx dt = zb(q) \\
& a'_1(q) = (1-zb(q))\int_{t=0}^{q} \int_{x=0}^{\infty} g(x,t)x dx dt + \int_{t=q}^{\infty} \int_{x=t-q}^{\infty} g(x,t)(x-(t-q)) dx dt \\
& a'_2(q) = (1-zb(q))\int_{t=0}^{q} \int_{x=0}^{\infty} g(x,t)x^2 dx dt + \int_{t=q}^{\infty} \int_{x=t-q}^{\infty} g(x,t)(x-(t-q))^2 dx dt \\
& \mathbb{E}[W'(q)] = b'(q) \left(\frac{a'_2(q)}{2a'_1(q)(1-\rho'_{2_q})} + \lambda'_2 F_p(q)\frac{\mathbb{E}[X(q)^2]}{2(1-\rho'_{2_q})^2}\right)  = zb(q) \left(\frac{a'_2(q)}{2a'_1(q)(1-z\rho'_{q})} + z\lambda F_p(q)\frac{\mathbb{E}[X(q)^2]}{2(1-z\rho'_{q})^2}\right)\\
& \mathbb{E}[R'(y)] = \int_{x=0}^{\infty} \frac{g(x,y)}{f_p(y)} \int_{t=0}^{x} \frac{dt}{1- \rho'_{2_{(y-t)^{+}}}} dx
\end{flalign*}




\begin{table}[h]
\centering
\caption{Models Comparison in terms of mean response time}
\label{tab:dataset_comparison}
\begin{tabular}{@{}lcc@{}}
\toprule
Job Predicted & Model 1 & Model 2\\ \midrule
Short & $\frac{\lambda \left(2- 2T^{1.5} K_3(2\sqrt{T}) \right)}{2\left(1-  \lambda \left(1- 2T K_2(2\sqrt{T} \right)\right)} + \mathbb{E}[S_1']$ & $ \frac{ \lambda \cdot \left( c_1^2 + 2c_1 \cdot (1- 2T K_2(2\sqrt{T})) + 2 - 2T^{1.5} K_3(2\sqrt{T})\right)}{2\left(1-\lambda(c_1 + 1- 2T K_2(2\sqrt{T})\right)} + \mathbb{E}[S_1']$ \\
Long & [TODO] & [TODO] \\
\bottomrule
\end{tabular}
\end{table}




#####

Abstract

In the realm of learning-augmented algorithms, integrating predictions from machine learning models to enhance algorithmic efficiency has been a focus of recent research. This paper delves into the practical application of these algorithms within queueing systems, particularly in scheduling scenarios. Prior studies have primarily investigated queues with predicted service times, but often overlook the resources and complexity involved in generating these predictions. Our work critically examines the cost implications of predictions in queueing systems, challenging the assumption that predictions are cost-free and external to the system's resources.

We introduce \alg{}, a novel scheduling policy designed for an M/G/1 queueing system. \alg{} employs a hierarchical approach to predictions, categorizing jobs into short and long based on one-bit "cheap predictions" and applying more detailed "expensive predictions" for longer jobs. This paper presents a comprehensive analysis of \alg{} in two distinct models: the external cost model and the server time cost model. Our findings offer insights into the trade-offs between the efficiency of prediction integration and the associated costs in real-world queueing systems, thus providing a deeper understanding of the practicality of learning-augmented algorithms in scheduling.

"Is It Worth Predicting? Introducing 'Frugal', a Cost-Efficient Scheduling Policy"

"Predict or Pass: Unveiling 'Frugal', the Smart Scheduling Innovator"

SkipCast

SkipPred

Predict or Pass - 

PrediChoice PrediGo



\begin{table}[h]
\centering
\caption{SOAP quantities comparison for predicted long with predicted size $q$ and actual size $x_J$}
\label{tab:model2_comparison}
{\tiny
\begin{tabularx}{\textwidth}{@{}lXX@{}}
\toprule
Quantity & Model 1 & Model 2 \\ \midrule
$\mathbb{E}[X^{\text{new}}]$ &\begin{multlined}[t]\int_{0}^{\infty} p_T(x) x f(x) dx + \int_{0}^{q-a} \int_{x = 0}^{\infty} x \cdot (1 - p_T(x)) g(x,y) dx dy\end{multlined}  &\begin{multlined}[t]\textcolor{blue}{c_1} + \int_{0}^{\infty} p_T(x) x f(x) dx  +  \textcolor{blue}{\int_{0}^{\infty} (1-p_T(x)) c_2 f(x) dx}  \\ + \int_{0}^{q-a_J} \int_{x = 0}^{\infty} (1 - p_T(x)) g(x,y) x  dx dy\end{multlined}  \\
$\mathbb{E}[X_0^{\text{old}}]$ &\begin{multlined}[t]\int_{0}^{\infty} p_T(x) x f(x) dx + \int_{0}^{q} \int_{x = 0}^{\infty} x \cdot (1 - p_T(x)) g(x,y) dx dy\end{multlined}  &\begin{multlined}[t]\textcolor{blue}{c_1} + \int_{0}^{\infty} p_T(x) x f(x) dx  +  \textcolor{blue}{\int_{0}^{\infty} (1-p_T(x)) c_2 f(x) dx}  \\ + \int_{0}^{q} \int_{x = 0}^{\infty} (1 - p_T(x)) g(x,y) x  dx dy\end{multlined}  \\
$\mathbb{E}[X_1^{\text{old}}]$ &\begin{multlined}[t] \int_{t = q}^{\infty} \int_{x = t-q}^{\infty} (1-p_T(x)) \cdot g(x, t)\cdot(x - (t - q))^2 \cdot dx dt\end{multlined}  &\begin{multlined}[t]\int_{t = q}^{\infty} \int_{x = t-q}^{\infty} (1-p_T(x)) \cdot g(x, t)\cdot(x - (t - q))^2 \cdot dx dt\end{multlined}  \\

\bottomrule
\end{tabularx}
}
\end{table}


\begin{table}[h]
\centering
\caption{SOAP quantities comparison for predicted short}
\label{tab:model2_comparison}
{\tiny
\begin{tabularx}{\textwidth}{@{}lXX@{}}
\toprule
Quantity & Model 1 & Model 2 \\ \midrule
$\mathbb{E}[X^{\text{new}}]$ &  $0$ & $0$  \\
$\mathbb{E}[X_0^{\text{old}}]$ & \begin{multlined}[t] \int_{0}^{\infty} p_T(x) x f(x) dx\end{multlined}  & \begin{multlined}[t] \textcolor{blue}{c_1} + \int_{0}^{\infty} p_T(x) x f(x) dx\end{multlined} \\
$\mathbb{E}[X_1^{\text{old}}]$ & $0$ & $0$ \\

\bottomrule
\end{tabularx}
}
\end{table}


\begin{table}[h]
\centering
\caption{Models Comparison in terms of mean response time}
\label{tab:dataset_comparison}
{\tiny
\begin{tabular}{@{}lcc@{}}
\toprule
Job Predicted & Model 1 & Model 2\\ \midrule
Short & $\frac{\lambda \left(2- 2T^{1.5} K_3(2\sqrt{T}) \right)}{2\left(1-  \lambda \left(1- 2T K_2(2\sqrt{T} \right)\right)} + \mathbb{E}[S_1']$ & $ \frac{ \lambda \cdot \left( c_1^2 + 2c_1 \cdot (1- 2T K_2(2\sqrt{T})) + 2 - 2T^{1.5} K_3(2\sqrt{T})\right)}{2\left(1-\lambda(c_1 + 1- 2T K_2(2\sqrt{T})\right)} + \mathbb{E}[S_1']$ \\
Long & [TODO] & [TODO] \\
\bottomrule
\end{tabular}
}
\end{table}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/rank_function_b_0_rank.png}
    \hspace{0.5cm} % Adds a space between the two figures
    \includegraphics[width=0.45\textwidth]{figs/rank_function_b_1_rank.png}
    \caption{Visual representation of exampled rank function $ rank(d, a) $ for (a) predicted long job ($b = 1$) (b) predicted short job ($b = 0$) (b). Each point combines the first component (class) and the second component (either $-a$ or $ r(x) - a $) into a single value, with the class component represented by color and the second component by position on the y-axis. This visualization demonstrates the relationship between the classes.}

\end{figure}




\rana{just between us -- to make sure we got SOAP right-- DELETE IN SUBMISSION}

SPRPT has a rank function $rank(r, a) = r - a$ for job of size $x$ and predicted size $r$, as this rank function is monotonic, $J$'s worst future rank is its initial prediction $r(x_J)=q$.

\[ rank_{d_J, x_J}^{\text{worst}} (a)= q -a\] where $q= r(x_J)$. When $a_J=0$, the rank function is denoted by $r_{worst}= rank_{d_J, x_J}^{\text{worst}} (0) = q$.


\subsubsection{$X^{\text{new}}[rank_{d_J, x_J}^{\text{worst}} (a)]$ computation:}
Suppose that a new job $K$ of predicted size $r(x_K)$ arrives when $J$ has age $a$. 
If $K$ has predicted job size less than $J$'s predicted remaining process time ($q - a$), $K$ will always outrank $J$. Thus


\[X_{x_K}^{new}[q - a]  = x_K \mathds{1}(r(x_K) < q - a)\]


\begin{align*}
\mathbb{E}[X^{new}[q - a]] = \int_{0}^{q-a} \int_{x_K = 0}^{\infty} x_K \cdot g(x_K,y) dx_K dy \\
\end{align*}


\subsubsection{$X_{0}^{\text{old}}[r_{worst}]$ computation:}
Whether job $I$ is an original or recycled job depends on its predicted size relative to J's predcited size.
If $r(x_I) \le q$, then $I$ is original until its completion because its rank never exceeds $q$.

\[
X_{0, x_I}^{\text{old}}[q] = x_I\mathds{1}(r(x_I) \le q)
\]



\begin{align*}
\mathbb{E}[X_{0}^{\text{old}}[q]] = \int_{y = 0}^{q} \int_{x_I = 0}^{\infty} x_I \cdot g(x_I,y) dx_I dy 
\end{align*}


\begin{align*}
\mathbb{E}[(X_{0}^{\text{old}}[q])^2]] = \int_{y = 0}^{q} \int_{x_I = 0}^{\infty} x_I^2 \cdot g(x_I, y) dx_I dy
\end{align*}







\subsubsection{$X_{i}^{\text{old}}[r_{worst}]$ computation:}
If $r(x_I) > q$, then $I$ starts out discarded but becomes recycled when $r(x_I) - a = q$. This means at age $a = r(x_I) -q$ and served till completion, which will be $x_I - a_I = x_I - (r(x_I) - q)$,  let $t = r(x_I)$:

Thus, we have:
\[
X_{1, x_I}^{\text{old}}[q] = x_I - (t - q)
\]
For $i \ge 2$, $$X_{i, x_I}^{\text{old}}[q] = 0$$



\begin{align*}
\mathbb{E}[X_{1}^{\text{old}}[q]^2] = \int_{t = q}^{\infty} \int_{x_I = t-q}^{\infty} g(x_I, t) \cdot (x_I - (t - q))^2 \cdot dx_I dt
\end{align*}



\subsubsection{Applying SOAP}
Applying Theorem 5.5 of SOAP~\cite{scully2018soap} yields that the mean response time of jobs with descriptor ($r(x_J)=q$) and size $x_J$ is:
Let
$$\rho'_q= \lambda \int_{y = 0}^{q} \int_{x_I = 0}^{\infty} x_I \cdot g(x_I,y) dx_I dy$$


\begin{align*}
\mathbb{E}[T(x_J, q)] = &\frac{\lambda \left(\int_{y = 0}^{q} \int_{x_I = 0}^{\infty} x_I^2\cdot  g(x_I, y) dx_I dy + \int_{t = q}^{\infty} \int_{x_I = t-q}^{\infty} g(x_I, t) \cdot(x_I - (t - q))^2 \cdot dx_I dt\right)}{2(1-\rho'_q)^2} \\
&+ \int_{0}^{x_J} \frac{1}{1-\rho'_{(q-a)^+}} \, da
\end{align*}



Let $f_p(y) = \int_{x=0}^{\infty} g(x,y) dx$, the mean response time for a job with size $x_J$ and any prediction is 
$$\mathbb{E}[T(x_J)] = \int_{y=0}^{\infty} f_p(y) \mathbb{E}[T(y, x_J)] dy$$


$$\mathbb{E}[T] = \int_{x=0}^{\infty} \int_{y=0}^{\infty} g(x,y)  \mathbb{E}[T(x,y)] dy dx$$


\rana{do the analysis also for server cost model}




\begin{figure*}[t]
	\begin{tabular}{ccc}
		\subfloat[cost vs. $\lambda$]{\includegraphics[width=\matrixCellWidth]{figs/graphs/model1/cost_vs_arrivalrate_perfectP.png}\label{fig:model1_perfectp_lambda}} &
		\subfloat[cost vs ratio]{\includegraphics[width = \matrixCellWidth]{figs/graphs/model1/cost_vs_ratio_perfectP_0_9.png}\label{fig:model1_perfectp_ratio}}  &
		\subfloat[cost vs T]{\includegraphics[width = \matrixCellWidth]{figs/graphs/model1/cost_vs_T_perfectP_0_9.png}} \\
	\end{tabular}
	\caption{Perfect predictor (a) $T=3$, $c_1=2$, $c_2=10$ (b) $\lambda = 0.9$, $c_1=2$, $T=3$ (c) $\lambda = 0.9$, $c_1=2$, $c_2=10$.}
	\label{fig:model1_perfectp}
\end{figure*}


\begin{figure}[h]
   \centering
   \includegraphics[width=0.7\linewidth]{figs/graphs/model1/time_vs_lambda_zeroprices.png}
   \caption{Mean response time vs. $\lambda$ when prices set to zero -- log scale, perfect prediction.}
   \label{fig:mean_reponse_time}
\end{figure}


\subsection{Sample for Cheap Prediction}
\begin{itemize}
    \item Our models first do cheap predictions for all jobs, then expensive predictions for long jobs. As another alternative, we can sample a subset of jobs for initial cheap predictions, followed by expensive predictions if needed. In the case of jobs not selected in the initial sampling, we directly use expensive predictions.

    \item If $c_1 == c_2$ -- there is no good prediction and better prediction, we can use the idea (we talked about it before) that runs each job for $T$ times, if it is short, done, otherwise return it back to the queue for prediction -- queue with feedback. In this case, we save the cheap prediction for each job and support fairness ( I'm not sure what is the exact definition of fairness in queueing, but I mean that even long jobs run for a defined time and not be punished of being long)
\end{itemize}


\rana{For perfect predictor it is:
$$\frac{\int_{x=T}^{\infty} f(x) \mathbb{E}[T(x, x)]_{ext}^{{PL}}  dx}{\int_{x=T}^{\infty} f(x) dx}$$}


We consider the setting of single queue with Poisson arrivals, service time exponentially distributed with mean 1 ($f(x) = e^{-x}$) and three prediction models: 1)






Perfect prediction, where job size prediction is the actual job size, with $p_T(x) = 1$ only if $x<T$, and $g(x,y) = e^{-x}$ 2) Exponential prediction model, where a prediction for a job with service time $x$ is itself exponentially distributed with mean $x$,  with $p_T(x) = 1 - e^{-(\frac{T}{x})}$, $g(x,y) = e^{\frac{-x-y}{x}}$ 3) Uniform prediction model, where a prediction for a job with service time $x$ is uniformly distributed between $(1-\alpha)x$ and $(1+\alpha)x$, so $g(x,y) = \frac{1}{2\alpha x}e^{-x}$ and $pT(x) = 0 \text{ if }  T \leq (1 - \alpha) x, \quad 1 \text{ if } T \geq (1 + \alpha) x, \quad \frac{T - (1 - \alpha) x}{2 \alpha x} \text{ otherwise}$.





\begin{figure*}[t]
	\begin{tabular}{ccc}
		\subfloat[cost vs ratio]{\includegraphics[width = \matrixCellWidth]{figs/graphs/model1/cost_vs_ratio_uniP_arrving_0.9_c1_0.5_t_1.png}\label{}}  &
		\subfloat[cost vs T]{\includegraphics[width = \matrixCellWidth]{figs/graphs/model1/cost_vs_T_uniP_arrving_0.9_c1_0.5_c2_2.0.png}} &
  		\subfloat[cost vs. $\lambda$]{\includegraphics[width=\matrixCellWidth]{figs/graphs/model1/cost_vs_arrivalrate_uniP_T_1.0_c1_0.5_c2_2.png}\label{fig:}} \\

	\end{tabular}
	\caption{Cost in the external model using uniform predictor ($\alpha = 0.5$), service times are exponentially distributed with mean 1 (a) cost vs. prices ratio when $\lambda = 0.9$, $c_1=0.5$, $T=1$ (b) cost vs. $T$ when $\lambda = 0.9$, $c_1=0.5$, $c_2=2$. (c) cost vs. arriving rate when $T=1$, $c_1=0.5$, $c_2=2$}
	\label{fig:model1_perfectp}
\end{figure*}





\begin{table}[h]
\centering
\caption{Policies comparison in terms of mean response time in the external cost model}
\label{tab:models_comparison}
{\tiny
\begin{tabularx}{\textwidth}{@{}lXX@{}}
\toprule
Policy & Predicted Short & Predicted Long\\ \midrule

\alg{} & $\frac{\lambda \mathbb{E}[{S'_{< T}}^2]}{2(1-\rho'_{<T})} + \mathbb{E}[S'_{< T}]$ &\begin{multlined}[t] \frac{\lambda}{2(1-\rho^{ext}_q)^2} \Bigg( \mathbb{E}[{S'_{<T}}^2] + \mathbb{E}[{S'_{\ge T, q}}^2] + a(q) \Bigg) + \\ \int_{0}^{x_J} \frac{1}{1-\rho^{ext}_{(q-a)^+}} \, da\end{multlined} \\



1bit & $\frac{\lambda \mathbb{E}[{S'_{< T}}^2]}{2(1-\rho'_{<T})} + \mathbb{E}[S'_{< T}]$ &\begin{multlined}[t] \frac{\lambda}{2(1-\rho)(1-\rho^{ext}_{new})} \mathbb{E}[{S}^2] + \int_{0}^{x_J} \frac{1}{1-\rho^{ext}_{new}} \, da \end{multlined}\\



SPRPT & - &\begin{multlined}[t] \frac{\lambda}{2(1-\rho'_q)^2} \Bigg(\int_{y = 0}^{q} \int_{x_I = 0}^{\infty} x_I^2\cdot  g(x_I, y) dx_I dy + \\ \int_{t = q}^{\infty} \int_{x_I = t-q}^{\infty} g(x_I, t) \cdot(x_I - (t - q))^2 \cdot dx_I dt\Bigg)
    + \int_{0}^{x_J} \frac{1}{1-\rho'_{(q-a)^+}} \, da \end{multlined}\\

\bottomrule
\end{tabularx}
}
\end{table}



\rana{edit to the server cost only}

\begin{table}[h]
\centering
\caption{Models Comparison of \alg{} and 1bit in terms of mean response time for predicted long jobs, these systems have the same response time for predicted short jobs}
\label{tab:models_comparison}
{\tiny
\begin{tabularx}{\textwidth}{@{}lXX@{}}
\toprule
Alg & External Cost& Server Cost\\ \midrule

\alg{} & \begin{multlined}[t] \frac{\lambda}{2(1-\rho^{ext}_q)^2} \Bigg( \mathbb{E}[{S'_{<T}}^2] + \mathbb{E}[{S'_{\ge T, q}}^2] + a(q) \Bigg) + \\ \int_{0}^{x_J} \frac{1}{1-\rho^{ext}_{(q-a)^+}} \, da\end{multlined}  & \begin{multlined}[t] \frac{\lambda}{2(1-\rho_{q}^{srv})^2} \cdot \Bigg(\mathbb{E}[{S''_{<T}}^2(c_1)] + (c_1 + c_2)^2 \cdot Q(T, q) + \mathbb{E}[{S''_{\ge T, q}}^2(c1 + c_2)]+ a(q)\Bigg) \\
 +\int_{0}^{x_J} \frac{1}{1-\rho_{(q-a)^+}^{srv}} da\end{multlined}\\



1bit & \begin{multlined}[t] \frac{\lambda}{2(1-\rho)(1-\rho^{ext}_{new})} \mathbb{E}[{S}^2] + \int_{0}^{x_J} \frac{1}{1-\rho^{ext}_{new}} \, da \end{multlined} & \begin{multlined}[t] \frac{\lambda}{2(1-\rho_{c_1})(1-\rho^{srv}_{new})} \int_{0}^{\infty} (x+c_1)^2 f(x) \, dx + \int_{0}^{x_J} \frac{1}{1-\rho^{srv}_{new}} \, da \end{multlined}  \\

\bottomrule
\end{tabularx}
}
\end{table}



\begin{table}[h]
\centering
\caption{Policies comparison in terms of mean response time in the external cost model}
\label{tab:models_comparison}
{\tiny
\begin{tabularx}{\textwidth}{@{}lXX@{}}
\toprule
Policy & Predicted Short & Predicted Long\\ \midrule

\alg{} & $\frac{\lambda \mathbb{E}[{S'_{< T}}^2]}{2(1-\rho'_{<T})} + \mathbb{E}[S'_{< T}]$ &\begin{multlined}[t] \frac{\lambda}{2(1-\rho^{ext}_q)^2} \Bigg( \mathbb{E}[{S'_{<T}}^2] + \mathbb{E}[{S'_{\ge T, q}}^2] + a(q) \Bigg) + \\ \int_{0}^{x_J} \frac{1}{1-\rho^{ext}_{(q-a)^+}} \, da\end{multlined} \\



1bit & $\frac{\lambda \mathbb{E}[{S'_{< T}}^2]}{2(1-\rho'_{<T})} + \mathbb{E}[S'_{< T}]$ &\begin{multlined}[t] \frac{\lambda}{2(1-\rho)(1-\rho^{ext}_{new})} \mathbb{E}[{S}^2] + \int_{0}^{x_J} \frac{1}{1-\rho^{ext}_{new}} \, da \end{multlined}\\



SPRPT & - &\begin{multlined}[t] \frac{\lambda}{2(1-\rho'_q)^2} \Bigg(\int_{y = 0}^{q} \int_{x_I = 0}^{\infty} x_I^2\cdot  g(x_I, y) dx_I dy + \\ \int_{t = q}^{\infty} \int_{x_I = t-q}^{\infty} g(x_I, t) \cdot(x_I - (t - q))^2 \cdot dx_I dt\Bigg)
    + \int_{0}^{x_J} \frac{1}{1-\rho'_{(q-a)^+}} \, da \end{multlined}\\

\bottomrule
\end{tabularx}
}
\end{table}




\begin{table}[h]
\centering
\caption{Models Comparison in terms of mean response time for predicted short and predicted long jobs}
\label{tab:models_comparison}
{\tiny
\begin{tabularx}{\textwidth}{@{}lXX@{}}
\toprule
Job Predicted & External Cost& Server Cost\\ \midrule
Short &  $\frac{\lambda \mathbb{E}[{S'_{< T}}^2]}{2(1-\rho'_{<T})} + \mathbb{E}[S'_{< T}]$ & $\frac{\lambda \cdot \left(c_1^2 + 2c_1 \mathbb{E}[S'_{<T}] + \mathbb{E}[{S'_{<T}}^2]\right)}{2(1-\rho_{PS}^{srv})} + \mathbb{E}[S'_{<T}]$  \\
Long & \begin{multlined}[t] \frac{\lambda}{2(1-\rho^{ext}_q)^2} \Bigg( \mathbb{E}[{S'_{<T}}^2] + \mathbb{E}[{S'_{\ge T, q}}^2] + a(q) \Bigg) \\ +  \int_{0}^{x_J} \frac{1}{1-\rho^{ext}_{(q-a)^+}} \, da\end{multlined}  & \begin{multlined}[t] \frac{\lambda}{2(1-\rho_{q}^{srv})^2} \cdot \Bigg(\mathbb{E}[{S''_{<T}}^2(c_1)] + (c_1 + c_2)^2 \cdot Q(T, q) + \mathbb{E}[{S''_{\ge T, q}}^2(c1 + c_2)]+ a(q)\Bigg) \\
 +\int_{0}^{x_J} \frac{1}{1-\rho_{(q-a)^+}^{srv}} da\end{multlined}\\

\bottomrule
\end{tabularx}
}
\end{table}


\begin{table}[h]
\centering
\caption{Models Comparison in terms of mean response time for predicted short and predicted long jobs}
\label{tab:models_comparison}
{\tiny
\begin{tabularx}{\textwidth}{@{}lXX@{}}
\toprule
Job Predicted & External Cost& Server Cost\\ \midrule
Short &  $\frac{\lambda \mathbb{E}[{S'_{< T}}^2]}{2(1-\rho'_{<T})} + \mathbb{E}[S'_{< T}]$ & $\frac{\lambda \cdot \left(c_1^2 + 2c_1 \mathbb{E}[S'_{<T}] + \mathbb{E}[{S'_{<T}}^2]\right)}{2(1-\rho_{PS}^{srv})} + \mathbb{E}[S'_{<T}]$  \\
Long & \begin{multlined}[t] \frac{\lambda}{2(1-\rho^{ext}_q)^2} \Bigg( \mathbb{E}[{S'_{<T}}^2] + \mathbb{E}[{S'_{\ge T, q}}^2] + a(q) \Bigg) \\ +  \int_{0}^{x_J} \frac{1}{1-\rho^{ext}_{(q-a)^+}} \, da\end{multlined}  & \begin{multlined}[t] \frac{\lambda}{2(1-\rho_{q}^{srv})^2} \cdot \Bigg(\mathbb{E}[{S''_{<T}}^2(c_1)] + (c_1 + c_2)^2 \cdot Q(T, q) + \mathbb{E}[{S''_{\ge T, q}}^2(c1 + c_2)]+ a(q)\Bigg) \\
 +\int_{0}^{x_J} \frac{1}{1-\rho_{(q-a)^+}^{srv}} da\end{multlined}\\

\bottomrule
\end{tabularx}
}
\end{table}


\colorbox{yellow}{
    \begin{minipage}{\textwidth}

case of uniform prediction:
\begin{align*}
    E[T(x,y)] = \frac{\lambda}{2 \cdot (1 - \rho''(y))^2} \Bigg( &\int_{0}^{x_{\text{upper limit}}} pT(x) \cdot x^2 \cdot f(x) \, dx \\
&+ \int_{0}^{x} (1 - pT(x)) \cdot x^2 \cdot f(x) \cdot \frac{y - (1 - \alpha) \cdot x}{2 \cdot \alpha \cdot x} \, dx \\
&+ \int_{y}^{y_{\text{upper limit}}} (1 - pT(x)) \cdot \left[ \int_{\max(y, (1-\alpha) \cdot x)}^{\min((1+\alpha) \cdot x, x_{\text{upper limit}})} g(x, t) \cdot (x - (t - y))^2 \, dt \right] \, dx \Bigg) \\
&+ \int_{0}^{x} \frac{1}{1 - \rho''(\max(0, y - a))} \, da
\end{align*}

$\rho''(q) = \lambda \left( \int_{0}^{x_{\text{upper limit}}} pT(x) \cdot x \cdot f(x) \, dx + \int_{0}^{x_{\text{upper limit}}} (1 - pT(x)) \cdot x \cdot f(x) \cdot \frac{q - (1 - \alpha) \cdot x}{2 \cdot \alpha \cdot x} \, dx \right)$
\end{minipage}
}





\begin{proof}
To analyze [X] in the [Y] cost model using SOAP, we first find the worst future rank and then calculate $X^{\text{new}}[rank_{d_J}^{\text{worst}} (a)]$, $X_{0}^{\text{old}}[r_{worst}]$ and $X_{i}^{\text{old}}[r_{worst}]$ for [Z} job.
For [Z] jobs, the rank function is monotonic as described in \eqref{eq:alg2_ext_rank_equation}, therefore J's worst future rank is its initial rank:
\[ rank_{d_J}^{\text{worst}} (a)=  \langle 2, -a \rangle \] and  $r_{worst}= rank_{d_J}^{\text{worst}} (0) = \langle 2, 0 \rangle$.



$X^{\text{new}}[rank_{d_J}^{\text{worst}} (a)]$:
Suppose that a new job $K$ arrives when $J$ has age $a_J$.
$J$'s delay due to $K$ depends on $K$ is predicted to be short or long. 

Only if $K$ is predicted short then it will preempt $J$ and be scheduled till completion because it has a higher class as long jobs are scheduled also according to FCFS so in case of $K$ predicted long it will not preempt $J$

\[X_{x_K}^{new}[\langle 2, - a \rangle]  = 
\begin{cases}
    x_K   & \text{$K$ is predicted short } \\
\end{cases}
\]


\begin{align*}
\mathbb{E}[X^{new}[\langle 2,- a \rangle]] = & \int_{0}^{\infty} p_T(x) x f(x) dx
\end{align*}


$X_{0}^{\text{old}}[r_{worst}]$:
Now old job $I$ either if predicted short or long is an original job then it remains original until its completion (regardless of if it is predicted long or short). Thus, for $i \ge 1$, $X_{i, x_I}^{\text{old}}[\langle 2, 0 \rangle] = 0$.


\[
X_{0, x_I}^{\text{old}}[\langle 2, 0 \rangle] = x_I
\]



\begin{align*}
\mathbb{E}[X_{0}^{\text{old}}[\langle 2, 0 \rangle]] = & \int_{0}^{\infty} x f(x) dx
\end{align*}


\begin{align*}
\mathbb{E}[(X_{0}^{\text{old}}[\langle 2, 0 \rangle])^2]] = &  \int_{0}^{\infty} x^2 f(x) dx
\end{align*}




Applying Theorem 5.5 of SOAP~\cite{scully2018soap} yields the result:
\begin{align*}
    \mathbb{E}[T(x_J)]_{ext}^{{PL}} = &\frac{\lambda}{2(1-\rho)(1-\rho^{ext}_{new})} \int_{0}^{\infty} x^2 f(x) \, dx + \int_{0}^{x_J} \frac{1}{1-\rho^{ext}_{new}} \, da
    \end{align*}
\end{align*}

Where $\rho^{ext}_{new} = \lambda \left(\int_{0}^{\infty} p_T(x) x f(x) dx \right)$.


\end{proof}



\newpage

\section{\algtwo{}}


%TODO: describe DelayPredict in details + the descriptor
%TODO: define a short job


{\bf MM:  need to explain what delay predict is -- e.g., We present an alterantive algorithm that ....;  need to explain $L$, etc.}

Rank function of \algtwo{}:
Here we assume that the service time prediction $r$ is greater than $L$, since jobs that require expensive prediction are longer than $L$. Since a job's age is $L$ when it is preempted and obtains a prediction, in the external model, the predicted remaining time for long jobs is $r-L - (a-L) = r-a$.  For the service time model their age after being predicted starts at $L+c_2$, so the predicted remaining time is $r-L - (a-L-c_2) = r-a -c_2$. Since $c_2$ is fixed among all jobs, instead of the predicted remaining time we can use $r-a$ as the rank for convenience.
Accordingly, \algtwo{} in the external cost model has the following rank function:


\begin{align}
\label{eq:alg2_ext_rank_equation}
rank_{ext}([x, r], a) = 
\begin{cases}
\langle 1, -a \rangle & \text{if }  0 \le a < L \\
\langle 2, r - a \rangle &  \text{ if } a \ge L
\end{cases}
\end{align}


In the server cost model, \algtwo{} results in the following rank function:
\begin{align}
\label{srv:alg2_rank_equation}
rank_{srv}([x, r], a) = 
\begin{cases}
\langle 1, -a \rangle & \text{if $0 \le a < L$ (initial rank)}, \\
\langle 2, -a \rangle & \text{if } a = L  \text{ (expensive prediction calculation)}, \\
\langle 3, r-a \rangle & \text{if } a > L + c_2  \text{ (long jobs after expensive prediction)}.
\end{cases}
\end{align}




\subsection{\algtwo{} in External Cost Model}



\begin{lemma}
\label{alg2_lemma_S_ext}
For \algtwo{} policy in both the external cost model and the server cost model, the expected mean response time for a short job of size $x_J$, $\mathbb{E}[T]_{ext}^{{\algtwo{}, S}}$ is


\begin{align*}
    \mathbb{E}[T]_{ext}^{{\algtwo{}, S}}  = &\frac{\lambda}{2(1-\rho_{L})} \Bigg(\int_{0}^{L} x^2 f(x) \, dx + \int_{L}^{\infty} L^2 f(x) dx \Bigg) + x_J
\end{align*}

Where $\rho_{L} = \lambda \left(\int_{0}^{L} x f(x) dx + \int_{L}^{\infty} L f(x) dx\right)$, the load due to jobs while limiting their sizes to $L$.

\end{lemma}




\begin{proof}
We first find the worst future rank and then calculate $X^{\text{new}}[rank_{d_J}^{\text{worst}} (a)]$, $X_{0}^{\text{old}}[r_{worst}]$ and $X_{i}^{\text{old}}[r_{worst}]$ for short jobs.
As both the external cost model and the server cost model treat short jobs the same, and their worst future rank is the same, the analysis holds for both.

For short jobs, the rank function is monotonic as described in \eqref{eq:alg2_ext_rank_equation}, therefore J's worst future rank is its initial rank:
\[ rank_{d_J}^{\text{worst}} (a)=  \langle 1, -a \rangle \] and  $r_{worst}= rank_{d_J}^{\text{worst}} (0) = \langle 1, 0 \rangle$.



$X^{\text{new}}[rank_{d_J}^{\text{worst}} (a)]$: Since short jobs have higher priorities than long jobs, and they are scheduled FCFS, nothing will preempt $J$; $X_{x_K}^{new}[\langle 1, - a \rangle]  = 0$


$X_{0}^{\text{old}}[r_{worst}]$:
If an old job $I$ is short, it remains original until it is completed. Otherwise, it remains original only for $L$ times. Thus, for $i \ge 1$, $X_{i, x_I}^{\text{old}}[\langle 1, 0 \rangle] = 0$ and


\[
X_{0, x_I}^{\text{old}}[\langle 1, 0 \rangle] =
\begin{cases}
    x_I   & \text{if $I$ is short} \\
    L & \text{if $I$ is long}
\end{cases}
\]


\begin{align*}
\mathbb{E}[X_{0}^{\text{old}}[\langle 1, 0 \rangle]] = & \int_{0}^{L} x f(x) dx + \int_{L}^{\infty} L f(x) dx
\end{align*}


\begin{align*}
\mathbb{E}[(X_{0}^{\text{old}}[\langle 1, 0 \rangle])^2]] = & \int_{0}^{L} x^2 f(x) dx + \int_{L}^{\infty} L^2 f(x) dx
\end{align*}




Applying Theorem 5.5 of SOAP~\cite{scully2018soap} yields the result:
\begin{align*}
    \mathbb{E}[T]_{ext}^{{\algtwo{}, S}}  = &\frac{\lambda}{2(1-\rho_{L})} \Bigg(\int_{0}^{L} x^2 f(x) \, dx + \int_{L}^{\infty} L^2 f(x) dx \Bigg) + x_J
\end{align*}

Where $\rho_{L} = \lambda \left(\int_{0}^{L} x f(x) dx + \int_{L}^{\infty} L f(x) dx\right)$.
\end{proof}






\begin{lemma}
\label{lemma_alg2_L_ext}
    For \algtwo{} policy in external cost model, the expected mean reponse time for a long job of true size $x_J$ and predicted size $q$ is

    \begin{align*}
    \mathbb{E}[T]_{ext}^{{\algtwo{}, L}}  = &\frac{\lambda}{2(1-\rho^{ext}_{L,q})^2} \Bigg(\int_{x=0}^{L} x^2 f(x) dx  \\
    &+ \int_{y = 0}^{q} \int_{x = L}^{\infty} x^2 \cdot g(x,y) dx dy + \int_{y = q}^{\infty} \int_{x = L}^{\infty} L^2 \cdot g(x,y) dx dy \\
    &+\int_{t = q}^{\infty} \int_{x =L+ t-q}^{\infty} g(x, t)\cdot(x -L- (t - q))^2 \cdot dx dt\Bigg) +  \int_{0}^{x_J} \frac{1}{1-\rho^{ext}_{L,(q-a)^+}} \, da
\end{align*}



Where $\rho^{ext}_{L, q} = \lambda \left(\int_{x=0}^{L} x f(x) dx + \int_{y = 0}^{q} \int_{x = L}^{\infty} x \cdot g(x,y) dx dy + \int_{y = q}^{\infty} \int_{x = L}^{\infty} L \cdot g(x,y) dx dy\right)$ is the load due to short jobs, long jobs predicted to be less than $q$, and other long jobs with their size limited at $L$. $(q-a)^+ = max(q-a, 0)$.


\end{lemma}


\begin{proof}


To analyze \algtwo{} for long job in the external cost model using SOAP, we first find the worst future rank and then calculate $X^{\text{new}}[rank_{d_J}^{\text{worst}} (a)]$, $X_{0}^{\text{old}}[r_{worst}]$ and $X_{i}^{\text{old}}[r_{worst}]$ for long job.
As described in \eqref{eq:alg2_ext_rank_equation}, the rank function for long jobs is monotonic, and every job's rank is strictly decreasing with age, thus $J$'s worst future rank is its initial rank, here: $rank_{d_J}^{\text{worst}} (a)=  \langle 2, q -a \rangle $ and $r_{worst}= rank_{d_J}^{\text{worst}} (0) = \langle 2, q \rangle$.



$X^{\text{new}}[rank_{d_J}^{\text{worst}} (a)]$:
Suppose that a new job $K$ of predicted size $r_K$ arrives when $J$ has age $a_J$.
$J$'s delay due to $K$ depends on whether $K$ is short or long. If $K$ is short then it will preempt $J$, since it has a higher priority, and be scheduled till completion. If $K$ is long and has a predicted job size less than $J$'s predicted remaining process time ($q - a_J$), $K$ will preempt $J$ and proceed until completion. Otherwise, If $K$ is long and has a predicted job size more than $J$'s predicted remaining process time, it will preempt $J$ but will be scheduled only for $L$ time.


Thus

\[X_{x_K}^{new}[\langle 2, q - a \rangle]  = 
\begin{cases}
    x_K   & \text{$K$ is short } \\
    x_K \mathds{1}(r_K < q - a) + L \cdot \mathds{1}(r_K \ge q - a) & \text{$K$ is long}
\end{cases}
\]


\begin{align*}
\mathbb{E}[X^{new}[\langle 2, q - a \rangle]] = & \int_{x=0}^{L} x f(x) dx + \int_{y = 0}^{q-a} \int_{x = L}^{\infty} x \cdot g(x,y) dx dy + \int_{y = q-a}^{\infty} \int_{x = L}^{\infty} L \cdot g(x,y) dx dy\\
\end{align*}


$X_{0}^{\text{old}}[r_{worst}]$:
Whether another job $I$ is an original or recycled job depends on whether it is short or long, and in the case it is long, it also depends on its predicted size relative to J's prediction.
If $I$ is short, then it remains original until its completion. Alternatively, if $I$ is long, it is original until completion if $r_I \le q$, otherwise it is original until $L$.

\[
X_{0, x_I}^{\text{old}}[\langle 2, q \rangle] = 
\begin{cases}
    x_K   & \text{$K$ is short } \\
    x_K \mathds{1}(r_K < q ) + L \cdot \mathds{1}(r_K \ge q ) & \text{$K$ is long}
\end{cases}
\]



\begin{align*}
\mathbb{E}[X_{0}^{\text{old}}[\langle 2, q \rangle]] = & \int_{x=0}^{L} x f(x) dx + \int_{y = 0}^{q} \int_{x = L}^{\infty} x \cdot g(x,y) dx dy + \int_{y = q}^{\infty} \int_{x = L}^{\infty} L \cdot g(x,y) dx dy
\end{align*}


\begin{align*}
\mathbb{E}[(X_{0}^{\text{old}}[\langle 2, q \rangle])^2]] = & \int_{x=0}^{L} x^2 f(x) dx + \int_{y = 0}^{q} \int_{x = L}^{\infty} x^2 \cdot g(x,y) dx dy + \int_{y = q}^{\infty} \int_{x = L}^{\infty} L^2 \cdot g(x,y) dx dy
\end{align*}




$X_{i}^{\text{old}}[r_{worst}]$:
If another job $I$ is long and if $r_I > q$, then $I$ starts out discarded but becomes recycled when $r_I - a = q$. This starts at age $a = r_I -q$ and continues until completion, which will be $x_I -L - a_I = x_I -L - (r_I - q)$. Thus, for $i \ge 2$, $X_{i, x_I}^{\text{old}}[\langle 2, q \rangle] = 0$. Let $t = r_I$:

\[
X_{1, x_I}^{\text{old}}[\langle 2, q \rangle] =
\begin{cases}
    0   & \text{if $I$ is short} \\
    x_I -L - (t - q) & \text{if $I$ is long}
\end{cases}
\]



\begin{align*}
\mathbb{E}[X_{1}^{\text{old}}[\langle 2, q \rangle]^2] = \int_{t = q}^{\infty} \int_{x =L+ t-q}^{\infty} g(x, t)\cdot(x -L- (t - q))^2 \cdot dx dt
\end{align*}



Applying Theorem~\ref{soaptheorem} leads to the result.

\begin{align*}
    \mathbb{E}[T]_{ext}^{{\algtwo{}, L}}  = &\frac{\lambda}{2(1-\rho^{ext}_{L,q})^2} \Bigg(\int_{x=0}^{L} x^2 f(x) dx + \int_{y = 0}^{q} \int_{x = L}^{\infty} x^2 \cdot g(x,y) dx dy + \int_{y = q}^{\infty} \int_{x = L}^{\infty} L^2 \cdot g(x,y) dx dy \\
    &+\int_{t = q}^{\infty} \int_{x =L+ t-q}^{\infty} g(x, t)\cdot(x -L- (t - q))^2 \cdot dx dt\Bigg) +  \int_{0}^{x_J} \frac{1}{1-\rho^{ext}_{L,(q-a)^+}} \, da
\end{align*}



Where $\rho^{ext}_{L, q} = \lambda \left(\int_{x=0}^{L} x f(x) dx + \int_{y = 0}^{q} \int_{x = L}^{\infty} x \cdot g(x,y) dx dy + \int_{y = q}^{\infty} \int_{x = L}^{\infty} L \cdot g(x,y) dx dy\right)$.

\end{proof}






\subsection{\algtwo{} in Server Cost Model}



\begin{lemma}
\label{lemma_alg2_L_srv}
    For \algtwo{} policy in the server cost model, the expected mean response time for a long job of true size $x_J$ and predicted size $q$ is
\begin{align*}
    \mathbb{E}[T]_{srv}^{{\algtwo{}, L}}  = &\frac{\lambda}{2(1-\rho^{srv}_{L,q})^2} \Bigg(\int_{x=0}^{L} x^2 f(x) dx + \int_{y = 0}^{q} \int_{x = L}^{\infty} (x+c_2)^2 \cdot g(x,y) dx dy \\
    & + \int_{y = q}^{\infty} \int_{x = L}^{\infty} (L + c_2)^2 \cdot g(x,y) dx dy \\
    &+\int_{t = q}^{\infty} \int_{x =L+ t-q}^{\infty} g(x, t)\cdot(x -L- (t - q))^2 \cdot dx dt\Bigg) +  \int_{0}^{x_J} \frac{1}{1-\rho^{srv}_{L,(q-a)^+}} \, da
\end{align*}



Where $\rho^{srv}_{L, q} = \lambda \left(\int_{x=0}^{L} x f(x) dx + \int_{y = 0}^{q} \int_{x = L}^{\infty} (x+c_2) \cdot g(x,y) dx dy + \int_{y = q}^{\infty} \int_{x = L}^{\infty} (L + c_2) \cdot g(x,y) dx dy\right)$.
is the load due to short jobs, long jobs predicted to be less than $q$, and other long jobs with their size limited at $L$. $(q-a)^+ = max(q-a, 0)$.


\end{lemma}



\begin{proof}
Now we calculate $X^{\text{new}}[rank_{d_J}^{\text{worst}} (a)]$, $X_{0}^{\text{old}}[r_{worst}]$ and $X_{i}^{\text{old}}[r_{worst}]$ for long jobs in the server cost most.

$X^{\text{new}}[rank_{d_J}^{\text{worst}} (a)]$:
$J$'s delay due to $K$ also depends on $K$ is short or long.
If $I$ is short, then it remains it is scheduled until its completion. Alternatively, if $I$ is long and $r_I \le q$ then it is scheduled until completion, otherwise it is scheduled until $L$.


\[X_{x_K}^{new}[\langle 3, q - a_J \rangle]  = 
\begin{cases}
    x_K   & \text{$K$ is short } \\
    (c_2 + x_K)\cdot \mathds{1}(r_K < q- a_J) + (c_2 + L) \cdot \mathds{1}(r_K \ge q- a_J) & \text{$K$ is long}
\end{cases}
\]


\begin{align*}
\mathbb{E}[X^{new}[\langle 3, q - a \rangle]] = & \int_{x=0}^{L} x f(x) dx + \int_{y = 0}^{q-a} \int_{x = L}^{\infty} (x+c_2) \cdot g(x,y) dx dy \\
& + \int_{y = q-a}^{\infty} \int_{x = L}^{\infty} (L + c_2) \cdot g(x,y) dx dy\\
\end{align*}


$X_{0}^{\text{old}}[r_{worst}]$:
The analysis is similar to the new arrival job. Whether another job $I$ is an original or recycled job depends on whether it is short or long, and in the case it is long, it also depends on its predicted size relative to J's prediction.



\[
X_{0, x_I}^{\text{old}}[\langle 3, q \rangle] = 
\begin{cases}
    x_K   & \text{$K$ is short } \\
    (c_2 + x_K)\cdot \mathds{1}(r_K < q) + (c_2 + L) \cdot \mathds{1}(r_K \ge q) & \text{$K$ is long}
\end{cases}
\]



\begin{align*}
\mathbb{E}[X_{0}^{\text{old}}[\langle 3, q \rangle]] =& \int_{x=0}^{L} x f(x) dx + \int_{y = 0}^{q} \int_{x = L}^{\infty} (x+c_2) \cdot g(x,y) dx dy + \int_{y = q}^{\infty} \int_{x = L}^{\infty} (L + c_2) \cdot g(x,y) dx dy\\
\end{align*}


\begin{align*}
\mathbb{E}[(X_{0}^{\text{old}}[\langle 3, q \rangle])^2]] = & \int_{x=0}^{L} x^2 f(x) dx + \int_{y = 0}^{q} \int_{x = L}^{\infty} (x+c_2)^2 \cdot g(x,y) dx dy \\
&+ \int_{y = q}^{\infty} \int_{x = L}^{\infty} (L + c_2)^2 \cdot g(x,y) dx dy\\
\end{align*}




$X_{i}^{\text{old}}[r_{worst}]$:
As described before, If another job $I$ is long and if $r_I > q$, then $I$ starts out discarded but becomes recycled when $r_I - a = q$. This starts at age $a = r_I -q$ and continues until completion, which will be $x_I -L - a_I = x_I -L - (r_I - q)$. Thus, for $i \ge 2$, $X_{i, x_I}^{\text{old}}[\langle 3, q \rangle] = 0$. Let $t = r_I$:

\[
X_{1, x_I}^{\text{old}}[\langle 3, q \rangle] =
\begin{cases}
    0   & \text{if $I$ is short} \\
    x_I -L - (t - q) & \text{if $I$ is long}
\end{cases}
\]



\begin{align*}
\mathbb{E}[X_{1}^{\text{old}}[\langle 3, q \rangle]^2] = \int_{t = q}^{\infty} \int_{x =L+ t-q}^{\infty} g(x, t)\cdot(x -L- (t - q))^2 \cdot dx dt
\end{align*}



Applying Theorem~\ref{soaptheorem} leads to the result.

\begin{align*}
    \mathbb{E}[T]_{srv}^{{\algtwo{}, L}}  = &\frac{\lambda}{2(1-\rho^{srv}_{L,q})^2} \Bigg(\int_{x=0}^{L} x^2 f(x) dx + \int_{y = 0}^{q} \int_{x = L}^{\infty} (x+c_2)^2 \cdot g(x,y) dx dy \\
    & + \int_{y = q}^{\infty} \int_{x = L}^{\infty} (L + c_2)^2 \cdot g(x,y) dx dy \\
    &+\int_{t = q}^{\infty} \int_{x =L+ t-q}^{\infty} g(x, t)\cdot(x -L- (t - q))^2 \cdot dx dt\Bigg) +  \int_{0}^{x_J} \frac{1}{1-\rho^{srv}_{L,(q-a)^+}} \, da
\end{align*}



Where $\rho^{srv}_{L, q} = \lambda \left(\int_{x=0}^{L} x f(x) dx + \int_{y = 0}^{q} \int_{x = L}^{\infty} (x+c_2) \cdot g(x,y) dx dy + \int_{y = q}^{\infty} \int_{x = L}^{\infty} (L + c_2) \cdot g(x,y) dx dy\right)$.

\end{proof}










\begin{restatable}{lemma}{lemmadelaypexts}
\label{lem:delayp_ext_s}
For \algtwo{} policy in both the external cost model and the server cost model, the expected mean response time for a short job, $\mathbb{E}[T]_{ext}^{{\algtwo{}, S}}$ is


\begin{align*}
    \mathbb{E}[T]_{ext}^{{\algtwo{}, S}} = \mathbb{E}[T]_{srv}^{{\algtwo{}, S}}  = &\frac{\lambda}{2(1-\rho_{L})} \Bigg(\int_{0}^{L} x^2 f(x) \, dx + \int_{L}^{\infty} L^2 f(x) dx \Bigg) + \int_{0}^{L} x f(x) dx
\end{align*}

Where $\rho_{L} = \lambda \left(\int_{0}^{L} x f(x) dx + \int_{L}^{\infty} L f(x) dx\right)$, the load due to jobs while limiting their sizes to $L$.

\end{restatable}




\begin{proof}
We first find the worst future rank and then calculate $X^{\text{new}}[rank_{d_J}^{\text{worst}} (a)]$, $X_{0}^{\text{old}}[r_{worst}]$ and $X_{i}^{\text{old}}[r_{worst}]$ for short jobs.
As both the external cost model and the server cost model treat short jobs the same, and their worst future rank is the same, the analysis holds for both.

For short jobs, the rank function is monotonic, therefore J's worst future rank is its initial rank:
\[ rank_{d_J}^{\text{worst}} (a)=  \langle 1, -a \rangle \] and  $r_{worst}= rank_{d_J}^{\text{worst}} (0) = \langle 1, 0 \rangle$.



$X^{\text{new}}[rank_{d_J}^{\text{worst}} (a)]$: Since short jobs have higher priorities than long jobs, and they are scheduled FCFS, a new job does not preempt $J$; $X_{x_K}^{new}[\langle 1, - a \rangle]  = 0$


$X_{0}^{\text{old}}[r_{worst}]$:
If an old job $I$ is short, it remains original until it is completed. Otherwise, it remains original only for $L$ times. Thus, for $i \ge 1$, $X_{i, x_I}^{\text{old}}[\langle 1, 0 \rangle] = 0$ and


\[
X_{0, x_I}^{\text{old}}[\langle 1, 0 \rangle] =
\begin{cases}
    x_I   & \text{if $I$ is short} \\
    L & \text{if $I$ is long}
\end{cases}
\]


\begin{align*}
\mathbb{E}[X_{0}^{\text{old}}[\langle 1, 0 \rangle]] = & \int_{0}^{L} x f(x) dx + \int_{L}^{\infty} L f(x) dx
\end{align*}


\begin{align*}
\mathbb{E}[(X_{0}^{\text{old}}[\langle 1, 0 \rangle])^2]] = & \int_{0}^{L} x^2 f(x) dx + \int_{L}^{\infty} L^2 f(x) dx
\end{align*}




Applying Theorem 5.5 of SOAP~\cite{scully2018soap} yields the result:
\begin{align*}
    \mathbb{E}[T]_{ext}^{{\algtwo{}, S}}  = &\frac{\lambda}{2(1-\rho_{L})} \Bigg(\int_{0}^{L} x^2 f(x) \, dx + \int_{L}^{\infty} L^2 f(x) dx \Bigg) + \int_{0}^{L} x f(x) dx
\end{align*}

Where $\rho_{L} = \lambda \left(\int_{0}^{L} x f(x) dx + \int_{L}^{\infty} L f(x) dx\right)$.
\end{proof}






\begin{restatable}{lemma}{lemmadelaypextl}
\label{lem:delayp_ext_l}
    For \algtwo{} policy in external cost model, the expected mean response time for a long job of true size $x_J$ and predicted size $q$ is

    \begin{align*}
    \mathbb{E}[T(x_J, q)]_{ext}^{{\algtwo{}, L}}  = &\frac{\lambda}{2(1-\rho^{ext}_{L,q})^2} \Bigg(\int_{x=0}^{L} x^2 f(x) dx  \\
    &+ \int_{y = 0}^{q} \int_{x = L}^{\infty} x^2 \cdot g(x,y) dx dy + \int_{y = q}^{\infty} \int_{x = L}^{\infty} L^2 \cdot g(x,y) dx dy \\
    &+\int_{t = q}^{\infty} \int_{x =L+ t-q}^{\infty} g(x, t)\cdot(x -L- (t - q))^2 \cdot dx dt\Bigg) +  \int_{0}^{x_J} \frac{1}{1-\rho^{ext}_{L,(q-a)^+}} \, da
\end{align*}



Where $\rho^{ext}_{L, q} = \lambda \left(\int_{x=0}^{L} x f(x) dx + \int_{y = 0}^{q} \int_{x = L}^{\infty} x \cdot g(x,y) dx dy + \int_{y = q}^{\infty} \int_{x = L}^{\infty} L \cdot g(x,y) dx dy\right)$ is the load due to short jobs, long jobs predicted to be less than $q$, and other long jobs with their size limited at $L$. $(q-a)^+ = max(q-a, 0)$.


\end{restatable}


\begin{proof}


To analyze \algtwo{} for long job in the external cost model using SOAP, we first find the worst future rank and then calculate $X^{\text{new}}[rank_{d_J}^{\text{worst}} (a)]$, $X_{0}^{\text{old}}[r_{worst}]$ and $X_{i}^{\text{old}}[r_{worst}]$ for long job.
As described in \eqref{eq:alg2_ext_rank_equation}, the rank function for long jobs is monotonic, and every job's rank is strictly decreasing with age, thus $J$'s worst future rank is its initial rank, here: $rank_{d_J}^{\text{worst}} (a)=  \langle 2, q -a \rangle $ and $r_{worst}= rank_{d_J}^{\text{worst}} (0) = \langle 2, q \rangle$.



$X^{\text{new}}[rank_{d_J}^{\text{worst}} (a)]$:
Suppose that a new job $K$ of predicted size $r_K$ arrives when $J$ has age $a_J$.
$J$'s delay due to $K$ depends on whether $K$ is short or long. If $K$ is short then it will preempt $J$, since it has a higher priority, and be scheduled till completion. If $K$ is long and has a predicted job size less than $J$'s predicted remaining process time ($q - a_J$), $K$ will preempt $J$ and proceed until completion. Otherwise, If $K$ is long and has a predicted job size more than $J$'s predicted remaining process time, it will preempt $J$ but will be scheduled only for $L$ time.


Thus

\[X_{x_K}^{new}[\langle 2, q - a \rangle]  = 
\begin{cases}
    x_K   & \text{$K$ is short } \\
    x_K \mathds{1}(r_K < q - a) + L \cdot \mathds{1}(r_K \ge q - a) & \text{$K$ is long}
\end{cases}
\]


\begin{align*}
\mathbb{E}[X^{new}[\langle 2, q - a \rangle]] = & \int_{x=0}^{L} x f(x) dx + \int_{y = 0}^{q-a} \int_{x = L}^{\infty} x \cdot g(x,y) dx dy + \int_{y = q-a}^{\infty} \int_{x = L}^{\infty} L \cdot g(x,y) dx dy\\
\end{align*}


$X_{0}^{\text{old}}[r_{worst}]$:
Whether another job $I$ is an original or recycled job depends on whether it is short or long, and in the case it is long, it also depends on its predicted size relative to J's prediction.
If $I$ is short, then it remains original until its completion. Alternatively, if $I$ is long, it is original until completion if $r_I \le q$, otherwise it is original until $L$.

\[
X_{0, x_I}^{\text{old}}[\langle 2, q \rangle] = 
\begin{cases}
    x_K   & \text{$K$ is short } \\
    x_K \mathds{1}(r_K < q ) + L \cdot \mathds{1}(r_K \ge q ) & \text{$K$ is long}
\end{cases}
\]



\begin{align*}
\mathbb{E}[X_{0}^{\text{old}}[\langle 2, q \rangle]] = & \int_{x=0}^{L} x f(x) dx + \int_{y = 0}^{q} \int_{x = L}^{\infty} x \cdot g(x,y) dx dy + \int_{y = q}^{\infty} \int_{x = L}^{\infty} L \cdot g(x,y) dx dy
\end{align*}


\begin{align*}
\mathbb{E}[(X_{0}^{\text{old}}[\langle 2, q \rangle])^2]] = & \int_{x=0}^{L} x^2 f(x) dx + \int_{y = 0}^{q} \int_{x = L}^{\infty} x^2 \cdot g(x,y) dx dy + \int_{y = q}^{\infty} \int_{x = L}^{\infty} L^2 \cdot g(x,y) dx dy
\end{align*}




$X_{i}^{\text{old}}[r_{worst}]$:
If another job $I$ is long and if $r_I > q$, then $I$ starts out discarded but becomes recycled when $r_I - a = q$. This starts at age $a = r_I -q$ and continues until completion, which will be $x_I -L - a_I = x_I -L - (r_I - q)$. Thus, for $i \ge 2$, $X_{i, x_I}^{\text{old}}[\langle 2, q \rangle] = 0$. Let $t = r_I$:

\[
X_{1, x_I}^{\text{old}}[\langle 2, q \rangle] =
\begin{cases}
    0   & \text{if $I$ is short} \\
    x_I -L - (t - q) & \text{if $I$ is long}
\end{cases}
\]



\begin{align*}
\mathbb{E}[X_{1}^{\text{old}}[\langle 2, q \rangle]^2] = \int_{t = q}^{\infty} \int_{x =L+ t-q}^{\infty} g(x, t)\cdot(x -L- (t - q))^2 \cdot dx dt
\end{align*}



Applying Theorem~\ref{soaptheorem} leads to the result.

\begin{align*}
    \mathbb{E}[T(x_J, q)]_{ext}^{{\algtwo{}, L}}  = &\frac{\lambda}{2(1-\rho^{ext}_{L,q})^2} \Bigg(\int_{x=0}^{L} x^2 f(x) dx \\
    &+ \int_{y = 0}^{q} \int_{x = L}^{\infty} x^2 \cdot g(x,y) dx dy + \int_{y = q}^{\infty} \int_{x = L}^{\infty} L^2 \cdot g(x,y) dx dy \\
    &+\int_{t = q}^{\infty} \int_{x =L+ t-q}^{\infty} g(x, t)\cdot(x -L- (t - q))^2 \cdot dx dt\Bigg) +  \int_{0}^{x_J} \frac{1}{1-\rho^{ext}_{L,(q-a)^+}} \, da
\end{align*}



Where $\rho^{ext}_{L, q} = \lambda \left(\int_{x=0}^{L} x f(x) dx + \int_{y = 0}^{q} \int_{x = L}^{\infty} x \cdot g(x,y) dx dy + \int_{y = q}^{\infty} \int_{x = L}^{\infty} L \cdot g(x,y) dx dy\right)$.

\end{proof}




\begin{restatable}{lemma}{lemmadelaypsrvl}
\label{lem:delayp_srv_l}
    For \algtwo{} policy in the server cost model, the expected mean response time for a long job of true size $x_J$ and predicted size $q$ is
\begin{align*}
    \mathbb{E}[T(x_J, q)]_{srv}^{{\algtwo{}, L}}  = &\frac{\lambda}{2(1-\rho^{srv}_{L,q})^2} \Bigg(\int_{x=0}^{L} x^2 f(x) dx + \int_{y = 0}^{q} \int_{x = L}^{\infty} (x+c_2)^2 \cdot g(x,y) dx dy \\
    & + \int_{y = q}^{\infty} \int_{x = L}^{\infty} (L + c_2)^2 \cdot g(x,y) dx dy \\
    &+\int_{t = q}^{\infty} \int_{x =L+ t-q}^{\infty} g(x, t)\cdot(x -L- (t - q))^2 \cdot dx dt\Bigg) +  \int_{0}^{x_J} \frac{1}{1-\rho^{srv}_{L,(q-a)^+}} \, da
\end{align*}



Where $\rho^{srv}_{L, q} = \lambda \left(\int_{x=0}^{L} x f(x) dx + \int_{y = 0}^{q} \int_{x = L}^{\infty} (x+c_2) \cdot g(x,y) dx dy + \int_{y = q}^{\infty} \int_{x = L}^{\infty} (L + c_2) \cdot g(x,y) dx dy\right)$.
is the load due to short jobs, long jobs predicted to be less than $q$, and other long jobs with their size limited at $L$ along with the load of the predictions. $(q-a)^+ = max(q-a, 0)$.


\end{restatable}



\begin{proof}
In this case, $J$'s worst future rank is $rank_{d_J}^{\text{worst}} (a)=  \langle 3, q -a \rangle $ and $r_{worst}= rank_{d_J}^{\text{worst}} (0) = \langle 3, q \rangle$. Now we calculate $X^{\text{new}}[rank_{d_J}^{\text{worst}} (a)]$, $X_{0}^{\text{old}}[r_{worst}]$ and $X_{i}^{\text{old}}[r_{worst}]$ for long jobs in the server cost most.

$X^{\text{new}}[rank_{d_J}^{\text{worst}} (a)]$:
$J$'s delay due to $K$ also depends on $K$ is short or long.
If $I$ is short, then it remains it is scheduled until its completion. Alternatively, if $I$ is long its prediction is scheduled for $c_2$. In addition, if $r_I \le q$ then it is scheduled until completion, otherwise it is scheduled until $L$.


\[X_{x_K}^{new}[\langle 3, q - a_J \rangle]  = 
\begin{cases}
    x_K   & \text{$K$ is short } \\
    (c_2 + x_K)\cdot \mathds{1}(r_K < q- a_J) + (c_2 + L) \cdot \mathds{1}(r_K \ge q- a_J) & \text{$K$ is long}
\end{cases}
\]


\begin{align*}
\mathbb{E}[X^{new}[\langle 3, q - a \rangle]] = & \int_{x=0}^{L} x f(x) dx + \int_{y = 0}^{q-a} \int_{x = L}^{\infty} (x+c_2) \cdot g(x,y) dx dy \\
& + \int_{y = q-a}^{\infty} \int_{x = L}^{\infty} (L + c_2) \cdot g(x,y) dx dy\\
\end{align*}


$X_{0}^{\text{old}}[r_{worst}]$:
The analysis is similar to the new arrival job. Whether another job $I$ is an original or recycled job depends on whether it is short or long, and in the case it is long, it also depends on its predicted size relative to J's prediction.



\[
X_{0, x_I}^{\text{old}}[\langle 3, q \rangle] = 
\begin{cases}
    x_K   & \text{$K$ is short } \\
    (c_2 + x_K)\cdot \mathds{1}(r_K < q) + (c_2 + L) \cdot \mathds{1}(r_K \ge q) & \text{$K$ is long}
\end{cases}
\]



\begin{align*}
\mathbb{E}[X_{0}^{\text{old}}[\langle 3, q \rangle]] =& \int_{x=0}^{L} x f(x) dx + \int_{y = 0}^{q} \int_{x = L}^{\infty} (x+c_2) \cdot g(x,y) dx dy + \int_{y = q}^{\infty} \int_{x = L}^{\infty} (L + c_2) \cdot g(x,y) dx dy\\
\end{align*}


\begin{align*}
\mathbb{E}[(X_{0}^{\text{old}}[\langle 3, q \rangle])^2]] = & \int_{x=0}^{L} x^2 f(x) dx + \int_{y = 0}^{q} \int_{x = L}^{\infty} (x+c_2)^2 \cdot g(x,y) dx dy \\
&+ \int_{y = q}^{\infty} \int_{x = L}^{\infty} (L + c_2)^2 \cdot g(x,y) dx dy\\
\end{align*}




$X_{i}^{\text{old}}[r_{worst}]$:
As described before, if another job $I$ is long and if $r_I > q$, then $I$ starts out discarded but becomes recycled when $r_I - a = q$. This starts at age $a = r_I -q$ and continues until completion, which will be $x_I -L - a_I = x_I -L - (r_I - q)$. Thus, for $i \ge 2$, $X_{i, x_I}^{\text{old}}[\langle 3, q \rangle] = 0$. Let $t = r_I$:

\[
X_{1, x_I}^{\text{old}}[\langle 3, q \rangle] =
\begin{cases}
    0   & \text{if $I$ is short} \\
    x_I -L - (t - q) & \text{if $I$ is long}
\end{cases}
\]



\begin{align*}
\mathbb{E}[X_{1}^{\text{old}}[\langle 3, q \rangle]^2] = \int_{t = q}^{\infty} \int_{x =L+ t-q}^{\infty} g(x, t)\cdot(x -L- (t - q))^2 \cdot dx dt
\end{align*}



Applying Theorem~\ref{soaptheorem} leads to the result.

\begin{align*}
    \mathbb{E}[T(x_J, q)]_{srv}^{{\algtwo{}, L}}  = &\frac{\lambda}{2(1-\rho^{srv}_{L,q})^2} \Bigg(\int_{x=0}^{L} x^2 f(x) dx + \int_{y = 0}^{q} \int_{x = L}^{\infty} (x+c_2)^2 \cdot g(x,y) dx dy \\
    & + \int_{y = q}^{\infty} \int_{x = L}^{\infty} (L + c_2)^2 \cdot g(x,y) dx dy \\
    &+\int_{t = q}^{\infty} \int_{x =L+ t-q}^{\infty} g(x, t)\cdot(x -L- (t - q))^2 \cdot dx dt\Bigg) +  \int_{0}^{x_J} \frac{1}{1-\rho^{srv}_{L,(q-a)^+}} \, da
\end{align*}



Where $\rho^{srv}_{L, q} = \lambda \left(\int_{x=0}^{L} x f(x) dx + \int_{y = 0}^{q} \int_{x = L}^{\infty} (x+c_2) \cdot g(x,y) dx dy + \int_{y = q}^{\infty} \int_{x = L}^{\infty} (L + c_2) \cdot g(x,y) dx dy\right)$.

\end{proof}




\begin{figure*}[t]
    \begin{tabular}{ccc}
        \subfloat[large cost gap, $c_1=0.5, c_2 = 2$]{\includegraphics[width = \matrixCellWidth]{figs/graphs/delaypredict/delayvsskip_cost_vs_arrivalrate_2p_exp_T_1.0_c1_0.5_c2_2.0_exp_lowcosts.png}\label{fig:delayp_lowcosts}} &
        \subfloat[small costs gap, $c_1=3.5, c_2 = 4$]{\includegraphics[width = \matrixCellWidth]{figs/graphs/delaypredict/delayvsskip_cost_vs_arrivalrate_2p_exp_T_1.0_c1_3.5_c2_4.0_exp_highcosts.png}\label{fig:delatp_hightcosts}} &
        \subfloat[cost vs. $\lambda$ - External]{\includegraphics[width=\matrixCellWidth]{figs/graphs/delaypredict/cost_vs_c1.png}\label{fig:ext_arriving}}
        \tabularnewline
        \multicolumn{3}{c}{\subfloat{\includegraphics[width=0.5\linewidth]{figs/graphs/delaypredict/delayp_legend.png}}}	

    \end{tabular}
    \caption{\rana{External cost model, exp dist, exp predictor} \rana{TODO: replace 1 with c1=0.5, c2=4..}}
    \label{fig:delaypredict}
\end{figure*}



==> singleQ_external.tex <==


\section{Single-Queue, External Cost}

We consider M/G/1 queueing system with arrival rate $\lambda$. The processing times for each arriving job are independent and drawn based on the cumulative distribution $F(x)$, with an associated density function $f(x)$.  Also associated with a job is an output from a binary predictor, $b$, which determines if a job is short or long, and for any job that is predicted to long, there is another output from a service-time predictor, $r$, which provides a real-number prediction of the service time for a job.  (If a job is predicted to be short, we do not consider $r$, and so we may take $r$ to be null.)  Hence a job is given by a triple $(x,b,r)$.  Here $b$ and $r$ will depend on $x$.
In particular, given a threshold $T$, the prediction $b$ is assumed to be independent over jobs, which a job being predicted as short (less than $T$) with probability $p_T(x)$. 
Similarly, the prediction $r$ is assumed to be independent over jobs, 
% and further the predictions $r$ and independent of the predictions $b$, 
and they are given by a density function $g(x,y)$, where $g(x,y)$ is the density corresponding to a job with actual size $x$ and predicted size $y$.  Hence
$$\int_{y=0}^\infty g(x,y) dy = f(x).$$


An interpretation of our model is that predictions are provided by an external server, with predicted long jobs going through an additional layer of prediction.  Accordingly, the predictions do not affect the service time of the job in this model. (Also, we treat the overall arrival process, still, as Poisson.) However, we do associate a cost with predictions.  All jobs obtain a binary prediction at some constant fixed cost $c_1$, called ``cheap prediction'', and all long jobs obtain a binary prediction at some fixed cost $c_2$, called ``expensive prediction''.
Accordingly, we can model the total expected cost for predictions per job in equilibrium as $C = c_1 + c_2 z$, where $z = \int f(x)(1-p_T(x))dx$ is the expected fraction of jobs requiring the second prediction.
In general, both $z$ and $c_1$ will depend on our choice of first layer prediction function, and similarly $c_2$ will depend on the choice of second layer prediction function. Therefore, for some parameterized families of prediction functions, we may wish to optimize our choice of predictors.
Specifically, letting $T$ be the expected response time for a job in the system in equilibrium, we might typically score a choice of predictors by the expected overall cost per job, which we model as some function $Q(C,T)$, such as a linear combination of the $C$ and $T$.

A practical approach prioritizes short jobs. In this system, short-predicted jobs are designated as non-preemptible and scheduled according to First-Come First-Served (FCFS). Jobs predicted to be long are considered preemptible and scheduled according to the Shortest Predicted Remaining Processing Time (SPRPT).
It can be viewed as a two-class priority system: Class 1 is for short jobs, managed by FCFS within the class. Class 2 is for long jobs, according to SPRPT using service time prediction, as we have this prediction for predicted long jobs.
Using SOAP~\cite{scully2018soap}, we can model the system using the descriptor $\mathcal{D} =$ [size, predicted short/long, predicted time] $ = [x, b, r(x)]$ and the following rank function:

\[
rank([x,b, r(x)], a) = 
\begin{cases}
\langle 1, -a \rangle & \text{if } b = 1 \\
\langle 2, r(x) - a \rangle &  \text{ if } b = 0
\end{cases}
\]




\begin{figure}[h]
   \centering
   \includegraphics[width=0.7\linewidth]{figs/model1_externalp.png}
   \caption{Single-queue, external cost overview. Note that there are two \emph{logical} queues, but they share a single physical queue in the sense that only one job is served at a time.}
   \label{fig:model_1_overview}
\end{figure}




\subsection{Mean response time}

Our model, as shown in Figure~\ref{fig:model_1_overview}, uses cheap predictions to categorize jobs into two groups: predicted short jobs and predicted long jobs. Predicted short jobs (scheduled according to FCFS) are referred to by $subsystem_1$ while predicted long jobs (scheduled according to SPRPT, which is based on predictions $r_i$) referred to by $subsystem_2$.

Each subsystem is analyzed separately. First, we compute the expected service times ($\mathbb{E}[S_1']$, and $\mathbb{E}[S_2']$), and the rate load ($\rho'_1$ and $\rho'_2$).


$$\mathbb{E}[S_1'] = \int_{0}^{\infty} x \cdot p_T(x) \cdot f(x) \, dx$$

$$\mathbb{E}[S_2'] = \int_{0}^{\infty} x \cdot (1 - p_T(x)) \cdot f(x) \, dx$$

$$\rho'_1= \lambda \int_{x=0}^{\infty} xf(x)p_T(x)\, dx$$
$$\rho'_2= \lambda \int_{x=0}^{\infty} xf(x)(1-p_T(x))\, dx$$


\subsection{Mean response time for predicted short job:}
While SOAP can be used to analyze the mean response time for predicted short jobs, this case is straightforward and follows the mean response time in the system for FCFS, which is given by $\mathbb{E}[T]^{FCFS} = \frac{\lambda \mathbb{E}[{S_1'}^2]}{2(1-\rho'_1)} + \mathbb{E}[S_1'] = \frac{\lambda \cdot  \int_{0}^{\infty} x^2 \cdot p_T(x) \cdot f(x) \, dx}{2(1-\lambda \int_{x=0}^{\infty} x \cdot p_T(x) \cdot f(x)\, dx)} +\int_{0}^{\infty} x \cdot p_T(x) \cdot f(x) \, dx$.

\colorbox{yellow}{
    \begin{minipage}{\textwidth}

For the setting with Poisson arrivals, service times are exponential with mean 1, and predicted service times are exponential with mean x when the actual service time
is x:
$f(x) = e^{-x}$, $p_T(x) = 1-e^{-\frac{T}{x}}$, $g(x,y) = \frac{1}{x} \cdot e^{\frac{-y}{x}}$.
In this setting, $\int f(x)p_T(x)dx = 1 - \int_{0}^{\infty} e^{-x-\frac{T}{x}}dx = 1- 2\sqrt{T}K_1(2\sqrt{T})$. Where $K_1$ is a modified Bessel function of the second kind.


$\rho'_1= \lambda \int_{x=0}^{\infty} xf(x)p_T(x)\, dx = \lambda \left(1- 2T K_2(2\sqrt{T} \right)$

$$\mathbb{E}[S_1'] = \int_{0}^{\infty} x \cdot p_T(x) \cdot f(x) \, dx = 1- 2T K_2(2\sqrt{T})$$

$$\mathbb{E}[S_1'^2] = \int_{0}^{\infty} x^2 \cdot p_T(x) \cdot f(x) \, dx = 2- 2T^{1.5} K_3(2\sqrt{T}$$

Thus:


\begin{equation*}
\mathbb{E}[T]^{FCFS} = \frac{\lambda \left(2- 2T^{1.5} K_3(2\sqrt{T}) \right)}{2\left(1-  \lambda \left(1- 2T K_2(2\sqrt{T} \right)\right)} + \mathbb{E}[S_1']
\end{equation*}



\end{minipage}
 }



\subsection{Mean response time for predicted long job:}
\rana{See appendix~\ref{appendix} for "pure" SPRPT analysis according to SOAP}

To calculate the mean response time of $subsystem_2$, we follow SOAP~\cite{scully2018soap} analysis.
Note that $subsystem_2$ has a monotonic rank function, and every job's rank is strictly decreasing with age, so J's worst future rank is its initial rank.
\[ rank_{d_J, x_J}^{\text{worst}} (a)=  \langle 2, q -a \rangle \] where $q= r(x_J)$. When $a_J=0$, the rank function is denoted by $r_{worst}= rank_{d_J, x_J}^{\text{worst}} (0) = \langle 2, q \rangle$.

Here, we calculate $X^{\text{new}}[rank_{d_J, x_J}^{\text{worst}} (a)]$, $X_{0}^{\text{old}}[r_{worst}]$ and $X_{i}^{\text{old}}[r_{worst}]$ for predicted long job.

\subsubsection{$X^{\text{new}}[rank_{d_J, x_J}^{\text{worst}} (a)]$ computation:}
Suppose that a new job $K$ of predicted size $r(x_K)$ arrives when $J$ has age $a_J$.
$J$'s delay due to $K$ depends on $K$ is predicted to be short or long. If $K$ is predicted short then it will preempt $J$ and be scheduled in $subsystem_1$ till completion because it has a higher class. Otherwise, if $K$ has a predicted job size less than $J$'s predicted remaining process time ($q - a_J$), $K$ will always outrank $J$. Thus

\[X_{x_K}^{new}[\langle 2, q - a \rangle]  = 
\begin{cases}
    x_K   & \text{$K$ is predicted short } \\
    x_K \mathds{1}(r(x_K) < q - a) & \text{$K$ is predicted long}
\end{cases}
\]


\begin{align*}
\mathbb{E}[X^{new}[\langle 2, q - a \rangle]] = & \int_{0}^{\infty} p_T(x) x f(x) dx + \int_{0}^{q-a} \int_{x = 0}^{\infty} x \cdot (1 - p_T(x)) g(x,y) dx dy \\
\end{align*}


\subsubsection{$X_{0}^{\text{old}}[r_{worst}]$ computation:}
Whether job $I$ is an original or recycled job depends on its prediction as short or long, and in the case of long, it also depends on its predicted size relative to J's prediction.
If $I$ is predicted short, then it remains original until its completion (regardless of its expensive prediction $r(x_I)$). Otherwise, if $I$ is predicted long, only if $r(x_I) \le q$, then $I$ is original until its completion because its rank never exceeds $q$.

\[
X_{0, x_I}^{\text{old}}[\langle 2, q \rangle] = 
\begin{cases}
    x_I   & \text{if $I$ is predicted short} \\
    x_I\mathds{1}(r(x_I) \le q) & \text{if $I$ is predicted long}
\end{cases}
\]



\begin{align*}
\mathbb{E}[X_{0}^{\text{old}}[\langle 2, q \rangle]] = & \int_{0}^{\infty} p_T(x) x f(x) dx + \int_{y = 0}^{q} \int_{x = 0}^{\infty} (1 - p_T(x)) \cdot x \cdot g(x,y) dx dy 
\end{align*}


\begin{align*}
\mathbb{E}[(X_{0}^{\text{old}}[\langle 2, q \rangle])^2]] = &  \int_{0}^{\infty} p_T(x) x^2 f(x) dx + \int_{y = 0}^{q} \int_{x = 0}^{\infty} (1-p_T(x)) \cdot x^2\cdot g(x, y) dx dy
\end{align*}







\subsubsection{$X_{i}^{\text{old}}[r_{worst}]$ computation:}
If $I$ is predicted long and if $r(x_I) > q$, then $I$ starts out discarded but becomes recycled when $r(x_I) - a = q$. This means at age $a = r(x_I) -q$ and served till completion, which will be $x_I - a_I = x_I - (r(x_I) - q)$.

Thus, we have:
\[
X_{1, x_I}^{\text{old}}[\langle 2, q \rangle] =
\begin{cases}
    0   & \text{if $I$ is predicted short} \\
    x_I - (r(x_I) - q) & \text{if $I$ is predicted long}
\end{cases}
\]
For $i \ge 2$, $$X_{i, x_I}^{\text{old}}[\langle 2, q \rangle] = 0$$
Let $t = r(x_I)$:


\begin{align*}
\mathbb{E}[X_{1}^{\text{old}}[\langle 2, q \rangle]^2] = \int_{t = q}^{\infty} \int_{x = t-q}^{\infty} (1-p_T(x)) \cdot g(x, t)\cdot(x - (t - q))^2 \cdot dx dt
\end{align*}



\subsubsection{Applying SOAP}
Applying Theorem 5.5 of SOAP~\cite{scully2018soap} yields that the mean response time of jobs with descriptor ($(b, r(x_J), x_J) = (1,q, x_J)$) and size $x_J$ is:
Let
$$\rho''_q= \lambda \left(\int_{0}^{\infty} p_T(x) x f(x) dx + \int_{y = 0}^{q} \int_{x = 0}^{\infty} (1 - p_T(x)) \cdot x \cdot g(x,y) dx dy \right)$$


\begin{align*}
\mathbb{E}[T(q, x_J)]^{SPRPT_{subsystem_2}} = &\frac{\lambda}{2(1-\rho''_q)^2} \Bigg( \int_{0}^{\infty} p_T(x) x^2 f(x) \, dx + \int_{y = 0}^{q} \int_{x = 0}^{\infty} (1-p_T(x)) x^2 g(x, y) \, dx \, dy \\
&\quad + \int_{t = q}^{\infty} \int_{x = t-q}^{\infty} (1-p_T(x)) g(x, t) (x - (t - q))^2 \, dx \, dt \Bigg) \\
&+ \int_{0}^{x_J} \frac{1}{1-\rho''_{(q-a)^+}} \, da
\end{align*}


Let $f_p(y) = \int_{x=0}^{\infty} g(x,y) dx$, the mean response time for a job with size $x_J$ and any prediction is 
$$\mathbb{E}[T(x_J)] = \int_{y=0}^{\infty} f_p(y) \mathbb{E}[T(y, x_J)]^{SPRPT_{subsystem_2}} dy$$

$$\mathbb{E}[T] = \int_{x=0}^{\infty} \int_{y=0}^{\infty} g(x,y) \mathbb{E}[T(0, y, x_J)] dy dx$$

\subsection{Total expected cost:}

We model the total expected cost as $$(1-z) \cdot \mathbb{E}[T]^{FCFS_{subsystem_1}} + z \cdot \mathbb{E}[T]^{SPRPT_{subsystem_2}} + C $$ where $z$ is the expected fraction of jobs requiring the second prediction and $C$ is the expected cost for prediction per job.



\subsection{Baselines}


\begin{figure*}[t]
	\begin{tabular}{ccc}
		\subfloat[cost vs. $\lambda$]{\includegraphics[width=\matrixCellWidth]{figs/graphs/model1/cost_vs_arrivalrate_perfectP.png}\label{fig:model1_perfectp_lambda}} &
		\subfloat[cost vs ratio]{\includegraphics[width = \matrixCellWidth]{figs/graphs/model1/cost_vs_ratio_perfectP_0_9.png}\label{fig:model1_perfectp_ratio}}  &
		\subfloat[cost vs T]{\includegraphics[width = \matrixCellWidth]{figs/graphs/model1/cost_vs_T_perfectP_0_9.png}} \\
	\end{tabular}
	\caption{Perfect predictor (a) $T=3$, $c_1=2$, $c_2=10$ (b) $\lambda = 0.9$, $c_1=2$, $T=3$ (c) $\lambda = 0.9$, $c_1=2$, $c_2=10$.}
	\label{fig:model1_perfectp}
\end{figure*}


\begin{figure}[h]
   \centering
   \includegraphics[width=0.7\linewidth]{figs/graphs/model1/time_vs_lambda_zeroprices.png}
   \caption{Mean response time vs. $\lambda$ when prices set to zero -- log scale, perfect prediction.}
   \label{fig:mean_reponse_time}
\end{figure}



As baselines, we compare our model to two single-queue models with external prediction. The first is expensive predictions for all jobs with SPRPT scheduling; this was previously studied~\cite{mitzenmacher2019scheduling}, in this case, the total expected cost is: $\mathbb{E}[T]^{SPRPT} + c_2 $ (See appendix~\ref{appendix} for $\mathbb{E}[T]^{SPRPT}$ analysis).



In our analysis, we focus on determining the conditions under which the following inequality holds true:
\begin{align*}
\mathbb{E}[T]^{SPRPT} + c_2 \ge (1-z) \cdot \mathbb{E}[T]^{FCFS_{subsystem_1}} + z \cdot \mathbb{E}[T]^{SPRPT_{subsystem_2}} + C
\end{align*}



%\begin{align*}
%\mathbb{E}[T] = &\frac{\lambda \left(\int_{y = 0}^{q} \int_{x_I = 0}^{\infty} x_I^2\cdot g(x_I, y) dx_I dy + \int_{t = q}^{\infty} \int_{x_I = t-q}^{\infty} g(x_I, t)\cdot(x_I - (t - q))^2 \cdot dx_I dt\right)}{2(1-\rho'_q)^2} \\
%&+ \int_{0}^{x_J} \frac{1}{1-\rho'_{(q-a)^+}} \, da
%\end{align*}





The second one is cheap predictions for all jobs with FCFS scheduling, as known as ``Queues with Small Advice''~\cite{mitzenmacher2021queues}, in this case, the total expected cost is: $$\mathbb{E}[T]^{FCFS} + c_1 $$



\rana{TODO: graph cost vs. T -- we should have similar cost with ($T=0$) or very small T's as with ~\cite{mitzenmacher2019scheduling}.
Graph2: cost vs. c2 c1 ratio. The cost affected by T and ratio}


\rana{based on the arrival rate $\lambda$, $c_1$ and $c_2$, you decide to set the threshold $T$ (on extreme $T=0$ is SRPT and }


\begin{comment}




The notations used in the last result for $\mathbb{E}[T]^{SPRPT}$ from~\cite{mitzenmacher2019scheduling} are:
$$f_p(y) = \int_{x=0}^{\infty} g(x,y) dx$$
$$\rho'_y = \lambda \int_{t=0}^{y} \int_{x=0}^{\infty} g(x,t) x dx dt$$

The following is known (see Section (4c) of~\cite{mitzenmacher2019scheduling}:
\begin{flalign}
& \mathbb{E}[T]^{SPRPT} = \int_{y=0}^{\infty} f_p(y)\mathbb{E}[W(y) + R(y)]dy  \label{eq_SPRPT} \\
& F_p(q) = \int_{x=0}^{q} f_p(x) dx \\
& \mathbb{E}[X(q)^2] = \frac{1}{F_p(q)} \int_{t=0}^{q} \int_{x=0}^{\infty} g(x,t) x^2 dx dt \\
& b(q) = \rho'_q + \lambda\int_{t=1}^{\infty} g(x,t)(x-(t-q))^{+} dx dt \\
& a_1(q) = (1-b(q))\int_{t=0}^{q} \int_{x=0}^{\infty} g(x,t)x dx dt + \int_{t=q}^{\infty} \int_{x=t-q}^{\infty} g(x,t)(x-(t-q)) dx dt \\
& a_2(q) = (1-b(q))\int_{t=0}^{q} \int_{x=0}^{\infty} g(x,t)x^2 dx dt + \int_{t=q}^{\infty} \int_{x=t-q}^{\infty} g(x,t)(x-(t-q))^2 dx dt \\
& \mathbb{E}[W(q)] = b(q) \left(\frac{a_2(q)}{2a_1(q)(1-\rho'_q)} + \lambda F_p(q)\frac{\mathbb{E}[X(q)^2]}{2(1-\rho'_q)^2}\right) \\
& \mathbb{E}[R(y)] = \int_{x=0}^{\infty} \frac{g(x,y)}{f_p(y)} \int_{t=0}^{x} \frac{dt}{1- \rho_{{(y-t)^{+}}}} dx
\end{flalign}

\subsection{Comments:}

- SOAP paper analyzes policies based on given descriptors and full information, not predicted descriptors. (replace $f(x)$ with $\int_{x=0}^{\infty} g(x,y)\,dx$ ? ) Can we write predictions over SOAP formulas? style of "price of misprediction" but more general?

- Consider $n$ jobs: $n_s$ short jobs and $n_l$ long jobs, two ways to analyze, 
(1) break it to 2 policies of the system, one FCFS of $n_s$ jobs with $n$ jobs of cheap predictions, the second of SPRPT with $n_l$ jobs and $n_l$ jobs of expensive predictions. Downside: no relation between the policies; that long jobs could be predicted while there are short jobs.

(2) one SOAP policy according to the above rank function, but take the mean according to $n$ (and not $2n+n_l$ and consider the prediction jobs as internal jobs). Downside: integrate predictions to SOAP formulas


SOAP policy of the whole system with


    \begin{figure}[h]
   \centering
   \includegraphics[width=0.7\linewidth]{figs/model2_servercost.png}
   \caption{Queue with feedback?, a combination of external arrivals (jobs) and internal predictions (predictions)}
   \label{fig:model3_overview}
\end{figure}


We start at $m=2$.
\[
f(x_i, m) = 
\begin{cases}
x_i & m = 1,4 \\
P_1(x_i) & m = 2 \\
P_2(x_i) & m = 3
\end{cases}
\]
\[
\text{next}(x_i, m) = 
\begin{cases}
m - 1 & P_1(x) \leq T \\
m + 1 & P_1(x) > T
\end{cases}
\]

\subsection{\rana{Comments}}
\begin{itemize}
    \item The arriving rate is not Poisson process (see Chapter 17.2), we can view that cheap predictions and short jobs/expensive prediction is a Poisson process (a job is expanded into two jobs at the arrivals but with different classes), but long prediction is not? 
    \item analysis: state representation (state = number of jobs in each class?),  write the balance equations considering the specific scheduling policy (these find the steady-state probabilities of each class?)? or we should use Jackson networks? (chapter 17)
\end{itemize}

Our prediction scheme is structured in a hierarchical manner with two sequential prediction layers.









If we want the expensive projections to be preemptible (by cheap predictions and by short jobs):
\begin{align*}
r([2,?],a) = \langle -a, 2\rangle\\
r([1,?],a) = \langle -a, 1\rangle\\
r([3,?],a) = \langle 3, -a\rangle\\
r([4,p(x)],a) = \langle 4, p(x) - a\rangle
\end{align*}


If we want the expensive projections to be nonpreemptible:
\begin{align*}
r([2,?],a) = \langle -a, 2\rangle\\
r([1,?],a) = \langle -a, 1\rangle\\
r([3,?],a) = \langle -a ,2\rangle\\
r([4,p(x)],a) = \langle 3, p(x) - a\rangle
\end{align*}



\end{comment}




==> singleQ_serverTime.tex <==
\section{Single-Queue, Server Time Cost}
We consider M/G/1 queueing system with arrival rate $\lambda$. The processing times for each arriving job are independent and drawn based on the cumulative distribution $F(x)$, with an associated density function $f(x)$.
Here, server time cost refers to the time taken by the server to make predictions. Within this framework, predictions are scheduled based on a defined rank function.


A reasonable policy might have predicated short jobs outrank other jobs. Note that to determine whether a job is short or long, it is initially scheduled for a "cheap prediction". Jobs predicted as short are categorized as non-preemptible while in execution, thereby prioritizing their completion before predicting new jobs. However, jobs predicted as long are further scheduled for a detailed "expensive prediction". Thus, cheap predictions outrank expensive predictions and long jobs. Similarly, expensive predictions are prioritized over predicted long jobs.

%{\bf MM:  Should explain here that we make short jobs non-preemptible when running, so predicting new jobs goes behind finishing predicted short jobs -- which makes sense, since even if the jobs were predicted short, they would go to the back of the "short job queue" -- hence the corresponding rank function.}
This hierarchical approach can be viewed as a four-class priority system: Class 1 is designated for short jobs, managed by FCFS within the class. Consequently, short jobs are non-preemptible, thus prioritizing them over predicting new ones. This approach is practical because even if the new jobs are predicted to be short, they are assigned behind the already running short jobs (Following FCFS). Class 2 includes jobs for cheap predictions, also operating under FCFS within their class. Class 3 involves jobs requiring expensive predictions, following the FCFS within the class. Finally, class 4 is reserved for long jobs, according to SPRPT using service time prediction from class 3. 

Following the framework of SOAP policies presented by Scully et al.~\cite{scully2018soap}, we can model the system using descriptor $\mathcal{D} =$ [size, predicted short/long, predicted time] $ = [x, b, r(x)]$ and the following rank function:


\[
rank([x,b, r(x)], a) = 
\begin{cases}
\langle 2, -a \rangle & \text{if $a = 0$ initial rank -- cheap prediction}, \\
\langle 1, -a \rangle & \text{if } b = 1 \text{ and } a > c_1 \text{ (after cheap prediction)}, \\
\langle 3, -a \rangle & \text{if } b = 0 \text{ and } a > c_1 \text{ (after cheap prediction -- expensive prediction)}, \\
\langle 4, r(x) - a \rangle &  \text{ if } b = 0 \text{ and } a > c_1 + c_2 \text{ (after expensive prediction)}.
\end{cases}
\]



\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/rank_function_b_0_rank.png}
    \hspace{0.5cm} % Adds a space between the two figures
    \includegraphics[width=0.45\textwidth]{figs/rank_function_b_1_rank.png}
    \caption{Visual representation of exampled rank function $ rank(d, a) $ for (a) predicted long job ($b = 1$) (b) predicted short job ($b = 0$) (b). Each point combines the first component (class) and the second component (either $-a$ or $ r(x) - a $) into a single value, with the class component represented by color and the second component by position on the y-axis. This visualization demonstrates the relationship between the classes.}

\end{figure}

\colorbox{yellow}{
    \begin{minipage}{\textwidth}
\textbf{simple case:}

For the setting with Poisson arrivals, service times are exponential with a mean of 1.
We consider the exponential prediction model where a prediction of a job with service time $x$ is itself exponentially distributed with mean $x$.
$$f(x) = e^{-x}$$
$$p_T(x) = 1-e^{-\frac{T}{x}}$$
$$g(x,y) = \frac{1}{x}e^{\frac{-y}{x}}$$

$$\int f(x)p_T(x)dx = 1 - \int_{0}^{\infty} e^{-x-\frac{T}{x}}dx = 1- 2\sqrt{T}K_1(2\sqrt{T})$$ Where $K_1$ is a modified Bessel function of the second kind.

$$\int xf(x)p_T(x)dx = \int_{0}^{\infty} xe^{-x} - xe^{-x-\frac{T}{x}}dx = 2- 2T K_2(2\sqrt{T})$$ Where $K_2$ is a modified Bessel function of the second kind (with different parameters).
\end{minipage}
}

\subsection{Mean response time analysis according to SOAP}
As explained, we first compute the worst future rank of $J$, denoted as $rank_{d_J, x_J}^{\text{worst}}$, as follows: 
\[ rank_{d_J, x_J}^{\text{worst}} (a)= \begin{cases} \langle 2, -a \rangle & \text{if $J$ is predicted short} \\ \langle 4, q -a\rangle & \text{if $J$ is predicted long} \end{cases} \]
where $q= r(x_J)$.
When $a_J=0$, the rank function is denoted by $r_{worst}= rank_{d_J, x_J}^{\text{worst}} (0)$.


We now proceed to the computation of $X^{\text{new}}[rank_{d_J, x_J}^{\text{worst}} (a)]$, $X_{0}^{\text{old}}[r_{worst}]$ and $X_{i}^{\text{old}}[r_{worst}]$ for predicted short job and for predicted long job.




\subsection{Mean response time for predicted short job:}

\subsubsection{$X^{\text{new}}[rank_{d_J, x_J}^{\text{worst}} (a)]$ computation:}
\label{sec:soap_x_new}

As mentioned, $X^{\text{new}}[rank_{d_J, x_J}^{\text{worst}} (a)]$ represents how long a new job that just arrived to the system is served until it completes or surpasses $rank_{d_J, x_J}^{\text{worst}} (a)$.
Let's consider a new job $K$ arriving when $J$ is at age $a_J$ (where $a_J \le \min(q, x_J)$). The worst rank of $J$ depends on whether $J$ is predicted to be short or long.
If $J$ is predicted short, then $J$'s worst future rank is its current rank $\langle 2, -a_J \rangle$. 
Given that $K$'s initial rank is $\langle 2, 0 \rangle$, at least equivalent to $J$'s worst future rank, the delay $J$ experiences due to $K$ is:
$$X_{x_K}^{new}[\langle 2, -a_J \rangle] = 0$$.



\subsubsection{$X_{0}^{\text{old}}[r_{worst}]$ computation:}
\label{sec:soap_x_0_old}

$X_{0}^{\text{old}}[r_{worst}]$ represents how long a job is served while its age is in its $0$-old $r_{worst}$-interval. This interval, as defined in SOAP (Definition 4.5), refers to the interval of ages during which a job is original with respect to rank $r_{worst}$.

We start by computing the relevant intervals according to our rank function. In our case, all jobs start with $\langle 2, 0 \rangle$ rank. Suppose that $J$ witnesses an old job $I$ of initial size $x_I$. The duration for which $I$ remains \emph{original} depends on whether its prediction is short or long.

if $J$ is predicted short, $r_{worst} = \langle 2, 0 \rangle$, if $I$ is also predicted short, its $0$-old $r_{worst}$-interval spans from $0$ to $\infty$, meaning that $I$ remains original until completion. Here, $X_{0}^{\text{old}}[r_{worst}] = c_1 + x_I$. Alternatively, if $I$ is predicted long, its $0$-old $r_{worst}$-interval is $[0, c_1]$, since after completing the cheap prediction phase (lasting $c_1$), its rank shifts to $\langle 3, 0 \rangle$. In this instance, $X_{0}^{\text{old}}[r_{worst}] = c_1$. Therefore, we have:

\[
X_{0, x_I}^{\text{old}}[\langle 2, 0 \rangle] = 
\begin{cases}
    c_1 + x_I   & \text{if $I$ is predicted short} \\
    c_1 & \text{if $I$ is predicted long}
\end{cases}
\]



\begin{align*}
\mathbb{E}[X_0^{\text{old}}[\langle 2, 0 \rangle]] =  c_1 + \int_{0}^{\infty} p_T(x) x f(x) dx
\end{align*}




\colorbox{yellow}{
\begin{minipage}{\textwidth}
\textbf{simple case:}
$$\mathbb{E}[X_0^{\text{old}}[\langle 2, 0 \rangle]] = c_1 + 1- 2T K_2(2\sqrt{T})$$
\end{minipage}
}



\begin{align*}
\mathbb{E}[X_0^{old}[\langle 2, 0 \rangle]^2]] =  \int_{0}^{\infty} p_T(x) (c_1 + x)^2 f(x) dx + \int_{0}^{\infty} (1-p_T(x)) \cdot c_1^2 \cdot f(x) dx \\
= c_1^2 + 2c_1 \int_{0}^{\infty} p_T(x) x f(x) dx + \int_{0}^{\infty} p_T(x) x^2 f(x) dx
\end{align*}

\colorbox{yellow}{
\begin{minipage}{\textwidth}
\textbf{simple case:}
\begin{align*}
\mathbb{E}[X_0^{old}[\langle 2, 0 \rangle]^2]] = c_1^2 + 2c_1 \cdot (1- 2T K_2(2\sqrt{T})) + \int_{0}^{\infty}(1-e^{\frac{-T}{x}}) e^{-x} x^2 dx \\
= c_1^2 + 2c_1 \cdot (1- 2T K_2(2\sqrt{T})) + \int_{0}^{\infty} x^2 e^{-x} dx - \int_{0}^{\infty} x^2 e^{-x-\frac{T}{x}} dx \\
= c_1^2 + 2c_1 \cdot (1- 2T K_2(2\sqrt{T})) + 2 - 2T^{1.5} K_3(2\sqrt{T}) \rana{recheck $K_3$..}
\end{align*}

\end{minipage}
}



\subsubsection{$X_{i}^{\text{old}}[r_{worst}]$ computation:}
\label{sec:soap_x_i_old}

For $i \ge 1$, $X_{i}^{\text{old}}[r_{worst}]$ represents how long a job is served while it is considered \emph{recycled} for the $i$ time with respect to the rank $r_{worst}$.

If $J$ is predicted short, $r_{worst} = \langle 2, 0 \rangle$, there are no instances of recycled jobs. This is because either $I$ completes its service (if predicted short) or it is discarded completely (if predicted long), and thus never gets a rank lower than $\langle 2, 0 \rangle$. As a result, for $i \ge 1$, $$X_{i, x_I}^{\text{old}}[\langle 2, 0 \rangle] = 0$$.



\subsubsection{Applying SOAP}

Let
\begin{itemize}
    \item $X_{PL}$ and $X_{PS}$ be the respective size distribution of predicted long jobs and predicted short jobs.
\end{itemize}

Applying Theorem 5.5 of SOAP~\cite{scully2018soap} yields that the mean response time of jobs with descriptor ($(b, *) = (1,*)$) -- predicted short jobs, and size $x_J$ is:

\begin{align*}
\mathbb{E}[T(1, *, x_J)] = & \frac{\lambda \cdot \mathbb{E}[X_0^{old}[\langle 2, 0 \rangle]^2]}{2(1-\lambda \mathbb{E}[X_0^{old}[\langle 2, 0 \rangle]]) (1-\lambda\mathbb{E}[X^{new}[\langle 2, 0 \rangle]])} + \int_{0}^{x_J} \frac{1}{1-\lambda\mathbb{E}[X^{new}[\langle 2, -a \rangle]]} da \\
& = \frac{\lambda \cdot \mathbb{E}[X_0^{old}[\langle 2, 0 \rangle]^2]}{2(1-\lambda \mathbb{E}[X_0^{old}[\langle 2, 0 \rangle]])} + \mathbb{E}[X_{PL}] = \frac{\lambda \cdot \mathbb{E}[X_0^{old}[\langle 2, 0 \rangle]^2]}{2(1-\rho_{0_{PS}}^{old})} + \mathbb{E}[X_{PL}]
\end{align*}

where $\rho_{0_{PS}}^{old} = \lambda \mathbb{E}[(X_0^{old}[\langle 2, 0 \rangle])$




\colorbox{yellow}{
\begin{minipage}{\textwidth}
\textbf{simple case:}

$\mathbb{E}[T(1, *, x_J)] = \frac{ \lambda \cdot ( c_1^2 + 2c_1 \cdot (1- 2T K_2(2\sqrt{T})) + 2 - 2T^{1.5} K_3(2\sqrt{T}))}{2(1-\lambda(c_1 + 1- 2T K_2(2\sqrt{T}))} + \mathbb{E}[X_{PL}]$
\end{minipage}
}

\colorbox{orange}{
\begin{minipage}{\textwidth}
\textbf{$\mathbb{E}[T(1, *, x_J)]$ analysis without SOAP theorem:}
If $J$ is predicted short, new arriving jobs do not preempt $J$. This is because if $J$ is undergoing its cheap prediction phase, it will, by FCFS during this phase, be queued ahead of the new job. Alternatively, if $J$ is already at the highest class (i.e., lowest rank), it will not be subject to preemption. As a result, the mean response time for $J$ is the sum of its waiting time and the size; \mathbb{E}[T_J] = \mathbb{E}[T_Q] + \mathbb{E}[X_J]$.

In addition, in this context, there are no recycled jobs, as discussed in Section~\ref{sec:soap_x_i_old}. This implies that the only delay $J$ experiences is from old jobs, equating to the waiting time in an FCFS system without server vacations, where the job size distribution in this scenario corresponds to $X_0^{\text{old}}[\langle 2, 0 \rangle]$.

To calculate the waiting time, we apply Equation 23.15 from~\cite{harchol2013performance}: $\mathbb{E}[T_Q] = \frac{\lambda \mathbb{E}[S^2]}{2(1-\rho)}$. By setting the job size distribution to $X_0^{\text{old}}[\langle 2, 0 \rangle]$, we can derive the desired result.
\end{minipage}
}




\subsection{Mean response time for predicted long job:}


\subsubsection{$X^{\text{new}}[rank_{d_J, x_J}^{\text{worst}} (a)]$ computation:}
\label{sec:soap_x_new}

If $J$ is predicted long, then $J$'s worst future rank is $\langle 4, r(x) - a_J\rangle$. In this case, $J$'s delay due to $K$ also depends on $K$ is predicted to be short or long.
\[X_{x_K}^{new}[\langle 4, q - a_J \rangle]  = 
\begin{cases}
    c_1 + x_K   & \text{$K$ is predicted short } \\
    c_1 + c_2 + x_K \mathds{1}(r(x_K) < q- a_J) & \text{$K$ is predicted long}
\end{cases}
\]


Employing the joint distribution $g(x,y)$, and setting $\mathds{1}(r(x_K) < q - a_J) = \int_{y=0}^{q - a_J} g(x_K,y) dy$, we can derive $J$'s expected delay due to any random new job:




\begin{align*}
\mathbb{E}[X^{new}[\langle 4, q - a_J \rangle]] = & c_1 + \int_{0}^{\infty} p_T(x) x f(x) dx +  \int_{0}^{\infty} (1-p_T(x)) c_2 f(x) dx\\
& + \int_{0}^{q-a_J} \int_{x = 0}^{\infty} (1 - p_T(x)) g(x,y) x  dx dy \\
\end{align*}




\colorbox{yellow}{
\begin{minipage}{\textwidth}
\textbf{simple case:}
$$\int xf(x)p_T(x)dx = \int_{0}^{\infty} xe^{-x} - xe^{-x-\frac{T}{x}}dx = 1- 2T K_2(2\sqrt{T})$$.

\begin{align*}
\int_{0}^{q-a_J} \int_{x = 0}^{\infty} (1 - p_T(x)) g(x,y) x  dx dy = \int_{0}^{q-a_J} \int_{x = 0}^{\infty} e^{\frac{-(T+y)}{x}}  dx dy
\end{align*}


\begin{align*}
    \mathbb{E}[X^{new}[\langle 4, q - a_J \rangle]] = c_1 + 1- 2T K_2(2\sqrt{T}) + c_2 \cdot 2\sqrt{T}K_1(2\sqrt{T}) + \int_{0}^{q-a_J} \int_{x = 0}^{\infty} e^{\frac{-(T+y)}{x}}  dx dy
\end{align*}
\end{minipage}
}


\subsubsection{$X_{0}^{\text{old}}[r_{worst}]$ computation:}
\label{sec:soap_x_0_old}

If $J$ is predicted long, $r_{worst} = \langle 4, q \rangle$. In this scenario, regardless of $I$'s prediction, the $0$-old $r_{worst}$-interval for $I$ spans from $0$ to $\infty$. This implies that $X_{0, x_I}^{\text{old}}[\langle 4, q \rangle]$ represents the entire service duration of $I$. Thus:

\[
X_{0, x_I}^{\text{old}}[\langle 4, q \rangle] = 
\begin{cases}
    c_1 + x_I   & \text{if $I$ is predicted short} \\
    c_1 + c_2 + x_I \cdot \mathds{1}(r(x_I) \le q) & \text{if $I$ is predicted long}
\end{cases}
\]





\begin{align*}
\mathbb{E}[X_{0}^{\text{old}}[\langle 4, q \rangle]] = & c_1 + \int_{0}^{\infty} p_T(x) x f(x) dx + \int_{0}^{\infty} (1-p_T(x)) c_2 f(x) dx \\
& + \int_{y = 0}^{q} \int_{x = 0}^{\infty} x \cdot (1 - p_T(x)) g(x,y)  dx dy \\
\end{align*}


\colorbox{yellow}{
\begin{minipage}{\textwidth}
\textbf{simple case:}
\begin{align*}
    \mathbb{E}[X_{0}^{\text{old}}[\langle 4, q \rangle]]  = c_1 + 1 - 2T K_2(2\sqrt{T}) + c_2 \cdot 2\sqrt{T}K_1(2\sqrt{T}) + \int_{0}^{q} \int_{x = 0}^{\infty} e^{\frac{-(T+y)}{x}}  dx dy
\end{align*}
\end{minipage}
}

\begin{align*}
\mathbb{E}[(X_{0}^{\text{old}}[\langle 4, q \rangle])^2]] = &  \int_{0}^{\infty} p_T(x) (c_1 + x)^2 f(x) dx + \int_{y = q}^{\infty} \int_{x = 0}^{\infty} (1-p_T(x)) \cdot g(x, y) \left(c_1 + c_2 \right)^2  dx dy \\
& + \int_{y = 0}^{q} \int_{x = 0}^{\infty} (1-p_T(x)) \cdot g(x, y) \left(c_1 + c_2 + x\right)^2  dx dy
\end{align*}





\colorbox{yellow}{
\begin{minipage}{\textwidth}
\textbf{simple case:}


\begin{align*}
    \mathbb{E}[(X_{0}^{\text{old}}[\langle 4, q \rangle])^2]] =  c_1^2 \left(1- 2\sqrt{T}K_1(2\sqrt{T})\right) + 2c_1 \cdot (1- 2T K_2(2\sqrt{T})) + 2 - 2T^{1.5} K_3(2\sqrt{T})  \\ + (c_1+c_2)^2 \int_{0}^{\infty} \frac{1}{x}e^{\frac{-(T+y)}{x}} dx dy +\int_{0}^{\infty} \frac{1}{x}e^{\frac{-(T+y)}{x}} \cdot \left(c_1 + c_2 + x\right)^2dx dy 
\end{align*}






\end{minipage}
}



\subsubsection{$X_{i}^{\text{old}}[r_{worst}]$ computation:}
\label{sec:soap_x_i_old}

If $J$ is predicted long, job $I$ may be recycled. This occurs when $I$ is predicted as long and with an expensive prediction $r(x_I) > q$. $I$ is initially considered as \emph{original} and is served during the cheap and expensive prediction phases, then discarded. At age $a_I = r(x_I) - q$, $I$ is recycled and served till completion, which will be $x_I - a_I = x_I - (r(x_I) - q)$.

Thus, we have:
\[
X_{1, x_I}^{\text{old}}[\langle 4, q \rangle] =
\begin{cases}
    0   & \text{if $I$ is predicted short} \\
    x_I - (r(x_I) - q) & \text{if $I$ is predicted long}
\end{cases}
\]
For $i \ge 2$, $$X_{i, x_I}^{\text{old}}[\langle 2, q \rangle] = 0$$

let $t = r(x_I)$

\begin{align*}
\mathbb{E}[X_{1}^{\text{old}}[\langle 4, q \rangle]^2] = \int_{t = q}^{\infty} \int_{x = t-q}^{\infty} (1-p_T(x)) \cdot g(x, t)\cdot(x - (t - q))^2 \cdot dx dt
\end{align*}

\colorbox{yellow}{
\begin{minipage}{\textwidth}
\textbf{simple case:}

\begin{align*}
    \mathbb{E}[X_{1}^{\text{old}}[\langle 4, q \rangle]^2] = \int_{t = q}^{\infty} \int_{x = t-q}^{\infty} e^{\frac{-(T+y)}{x}} \cdot(x - (t - q))^2 \cdot dx dt
\end{align*}

\end{minipage}
}


\subsubsection{Applying SOAP}

Let
\begin{itemize}
    \item $X_{PL}$ and $X_{PS}$ be the respective size distribution of predicted long jobs and predicted short jobs.
\end{itemize}

Applying Theorem 5.5 of SOAP~\cite{scully2018soap} yields that the mean response time of jobs with descriptor ($(b, r(x_J)) = (0,q)$) -- predicted long jobs with predicted size $q$, and actual size $x_J$ is:


\begin{align*}
\mathbb{E}[T(0, q, x_J)] =  & \frac{\lambda \cdot (\mathbb{E}[X_0^{old}[\langle 4, q \rangle]^2] + \mathbb{E}[X_1^{old}[\langle 4, q \rangle]^2])}{2(1-\lambda \mathbb{E}[X_0^{old}[\langle 4, q \rangle]) (1-\lambda\mathbb{E}[X^{new}[\langle 4, q \rangle])} \\
& +\int_{0}^{x_J} \frac{1}{1-\lambda\mathbb{E}[X^{new}[\langle 4, q - a \rangle]]} da
\end{align*}


Let $f_p(y) = \int_{x=0}^{\infty} g(x,y) dx$, the mean response time for a job with size $x_J$ and any prediction is 
$$\mathbb{E}[T(x_J)] = \int_{y=0}^{\infty} f_p(y) \mathbb{E}[T(0, y, x_J)] dy$$


\rana{$$\mathbb{E}[T] = \int_{y=0}^{\infty} \frac{g(x,y)}{f_p(y)}\int_{y=0}^{\infty} f_p(y) \mathbb{E}[T(0, y, x_J)] dy dx$$ ??}


\colorbox{orange}{
\begin{minipage}{\textwidth}
\textbf{$\mathbb{E}[T_{x_J\text{- predicted long with size $x_J$}}]$ analysis without SOAP theorem:}
If $J$ is predicted long, the delay from newly arriving jobs is incorporated into $J$'s waiting time. We approach the analysis of $J$'s waiting time by considering the length of the busy period for new arrivals, characterized by a job size distribution $X^{\text{new}}[\langle 4, q \rangle]$. This period begins with an initial workload $W$, representing an old jobs delay.

As shown in Equation 27.7 from~\cite{harchol2013performance}, the mean length of this busy period is given by $\mathbb{E}[B_W] = \frac{\mathbb{E}[W]}{1-\rho_{\text{new}}} = \frac{\mathbb{E}[W]}{1-\lambda \mathbb{E}[X^{\text{new}}[\langle 4, q \rangle]]}$. This workload $W$ is equivalent to the waiting time in an FCFS system with server vacations, where jobs arrive at rate $\lambda$ and have a size distribution $X_0^{\text{old}}[\langle 4, q \rangle]$.

In our model, we consider a single type of vacation, the length of which is determined by the distribution $X_1^{\text{old}}[\langle 4, q \rangle]$ (see section~\ref{sec:soap_x_i_old}). Following Section 27.2 in~\cite{harchol2013performance}, the Laplace-Stieltjes transform of the waiting time in an M/G/1 queue with vacations of length $V$ is $\tilde{T}^{M/G/1/\text{Vac}}(s) = \tilde{T}^{M/G/1}(s) \cdot \tilde{V_e}(s)$, where $\tilde{V_e}(s)$ is the excess of $V$. Therefore, the expected total time in an M/G/1 queue with vacations is $E[T]^{M/G/1/\text{Vac}} = E[T]^{M/G/1} + E[V_e]$. --\rana{recheck.}

To compute $E[T]^{M/G/1/\text{Vac}}$, we use Equation 23.15 from~\cite{harchol2013performance}: $\mathbb{E}[T_Q] = \frac{\lambda \mathbb{E}[S^2]}{2(1-\rho)}$, applying the job size distribution $X_0^{\text{old}}[\langle 4, q \rangle]$ for this calculation.

For the calculation of $V_e$, we refer to Equation 23.15 from~\cite{harchol2013performance}
....
\end{minipage}
}


\colorbox{yellow}{
\begin{minipage}{\textwidth}
\textbf{simple case:}

\mathbb{E}[T_{x_J\text{- predicted long with size $x_J$}}]  = 






\end{minipage}
}




\begin{comment}
Cheap predictions is uniform prediction model: predictions are uniformly distributed between 0 and a maximum value $M$ ($T \le M$). The formula for $ p_T(x) $ is:
$p_T(x) = \frac{T}{M} $
Expensive prediction is a linear prediction model: The predicted size $ y $ is a fixed proportion $ k $ of the actual size $ x $. The joint density function $ g(x, y) $ is:
\begin{equation}
g(x, y) = e^{-x} \cdot \delta(y - kx)
\end{equation}
In this setting, ....
\end{comment}

\subsection{Total Expected Cost}
We model the total expected cost as $$(1-z) \cdot \mathbb{E}[T_{x_J\text{- predicted long}}] + z \cdot \mathbb{E}[T_{x_J\text{- predicted long}}] $$ 


%calc second moment of x_0_old, x_1_old, 
% calc soap equations
%derive equations without SOAP..
% simple example to verify


%===============


\subsection{Baselines}

As baselines, we compare our model to two single-queue models with service time to compute the predictions. These models are preemptive, running either expensive predictions for all jobs with SPRPT or cheap predictions for all jobs with FCFS.


\section{Model 1 and 2 comparison}




\begin{table}[h]
\centering
\caption{SOAP quantities comparison for predicted long with predicted size $q$ and actual size $x_J$}
\label{tab:model2_comparison}
{\tiny
\begin{tabularx}{\textwidth}{@{}lXX@{}}
\toprule
Quantity & Model 1 & Model 2 \\ \midrule
$\mathbb{E}[X^{\text{new}}]$ &\begin{multlined}[t]\int_{0}^{\infty} p_T(x) x f(x) dx + \int_{0}^{q-a} \int_{x = 0}^{\infty} x \cdot (1 - p_T(x)) g(x,y) dx dy\end{multlined}  &\begin{multlined}[t]\textcolor{blue}{c_1} + \int_{0}^{\infty} p_T(x) x f(x) dx  +  \textcolor{blue}{\int_{0}^{\infty} (1-p_T(x)) c_2 f(x) dx}  \\ + \int_{0}^{q-a_J} \int_{x = 0}^{\infty} (1 - p_T(x)) g(x,y) x  dx dy\end{multlined}  \\
$\mathbb{E}[X_0^{\text{old}}]$ &\begin{multlined}[t]\int_{0}^{\infty} p_T(x) x f(x) dx + \int_{0}^{q} \int_{x = 0}^{\infty} x \cdot (1 - p_T(x)) g(x,y) dx dy\end{multlined}  &\begin{multlined}[t]\textcolor{blue}{c_1} + \int_{0}^{\infty} p_T(x) x f(x) dx  +  \textcolor{blue}{\int_{0}^{\infty} (1-p_T(x)) c_2 f(x) dx}  \\ + \int_{0}^{q} \int_{x = 0}^{\infty} (1 - p_T(x)) g(x,y) x  dx dy\end{multlined}  \\
$\mathbb{E}[X_1^{\text{old}}]$ &\begin{multlined}[t] \int_{t = q}^{\infty} \int_{x = t-q}^{\infty} (1-p_T(x)) \cdot g(x, t)\cdot(x - (t - q))^2 \cdot dx dt\end{multlined}  &\begin{multlined}[t]\int_{t = q}^{\infty} \int_{x = t-q}^{\infty} (1-p_T(x)) \cdot g(x, t)\cdot(x - (t - q))^2 \cdot dx dt\end{multlined}  \\

\bottomrule
\end{tabularx}
}
\end{table}


\begin{table}[h]
\centering
\caption{SOAP quantities comparison for predicted short}
\label{tab:model2_comparison}
{\tiny
\begin{tabularx}{\textwidth}{@{}lXX@{}}
\toprule
Quantity & Model 1 & Model 2 \\ \midrule
$\mathbb{E}[X^{\text{new}}]$ &  $0$ & $0$  \\
$\mathbb{E}[X_0^{\text{old}}]$ & \begin{multlined}[t] \int_{0}^{\infty} p_T(x) x f(x) dx\end{multlined}  & \begin{multlined}[t] \textcolor{blue}{c_1} + \int_{0}^{\infty} p_T(x) x f(x) dx\end{multlined} \\
$\mathbb{E}[X_1^{\text{old}}]$ & $0$ & $0$ \\

\bottomrule
\end{tabularx}
}
\end{table}


\begin{table}[h]
\centering
\caption{Exponential prediction case: Models Comparison in terms of mean response time}
\label{tab:dataset_comparison}
\begin{tabular}{@{}lcc@{}}
\toprule
Job Predicted & Model 1 & Model 2\\ \midrule
Short & $\frac{\lambda \left(2- 2T^{1.5} K_3(2\sqrt{T}) \right)}{2\left(1-  \lambda \left(1- 2T K_2(2\sqrt{T} \right)\right)} + \mathbb{E}[S_1']$ & $ \frac{ \lambda \cdot \left( c_1^2 + 2c_1 \cdot (1- 2T K_2(2\sqrt{T})) + 2 - 2T^{1.5} K_3(2\sqrt{T})\right)}{2\left(1-\lambda(c_1 + 1- 2T K_2(2\sqrt{T})\right)} + \mathbb{E}[S_1']$ \\
Long & [TODO] & [TODO] \\
\bottomrule
\end{tabular}
\end{table}

==> soap_analysis.tex <==
\section{Mean response time analysis according to SOAP}
In our analysis of the mean response time, we follow the SOAP approach~\cite{scully2018soap}. This analysis uses the tagged-job technique. We focus on a specific job, the 'tagged job', denoted by J, of size $x_J$ and descriptor $d_J$. The mean response time of $J$ is given by the sum of the residence time and the waiting time. To calculate the waiting time, we consider the delays caused by other jobs in the system with $J$. There are two key components: first, determining the delay caused by each ``new'' job (those arriving after J, each denoted by $K$); and second, determining the delay caused by ``old'' jobs (those arriving before J, each denoted by $I$).


First, to account for the nonmonotonic rank function, we first compute the worst future rank of $J$, denoted as $rank_{d_J, x_J}^{\text{worst}}$
When $a_J=0$, the rank function is denoted by $r_{worst}= rank_{d_J, x_J}^{\text{worst}} (0)$.

In the SOAP framework, waiting time is defined as equivalent to the transformed busy period in an M/G/1 system with arrival rate $\lambda$ and job size $X^{\text{new}}[rank_{d_J, x_J}^{\text{worst}} (a)]$ \footnote{$X^{\text{new}}[rank_{d_J, x_J}^{\text{worst}} (a)]$ represents how long a new job that just arrived to the system is served until it completes or surpasses $rank_{d_J, x_J}^{\text{worst}} (a)$}(defined and calculated in section~\ref{sec:soap_x_new}). The initial work of this period represents the delay caused by old jobs.

To deal with the delay due to old jobs, SOAP introduced a transformed system where jobs are categorized based on their rank. \emph{Discarded} old jobs, exceeding the rank threshold $r_{worst}$, are excluded from the transformed system. \emph{Original} old jobs, with a rank at or below $r_{worst}$, are considered as arrivals with rate $\lambda$ and a specific size distribution $X_{0}^{\text{old}}[r_{worst}]$ \footnote{$X_{0}^{\text{old}}[r_{worst}]$ represents how long a job is served while it is considered \emph{original} with respect to the rank $r_{worst}$} (defined and calculated in section~\ref{sec:soap_x_0_old}). \emph{Recycled old jobs}, currently at or below $r_{worst}$ but previously above this threshold, are treated as server vacations of length $X_{i}^{\text{old}}[r_{worst}]$\footnote{$X_{i}^{\text{old}}[r_{worst}]$ represents how long a job is served while it is considered \emph{recycled} for the $i$ time with respect to the rank $r_{worst}$} for $i \ge 1$ (defined and calculated in section~\ref{sec:soap_x_i_old}) in the transformed system.

SOAP shows that, because Poisson arrivals see time averages, the stationary delay due to old jobs has the same distribution as queueing time in the transformed M/G/1/FCFS system. This system is characterized by 'sparse' server vacations, where (\emph{original}) jobs arrive at rate $\lambda$ and follow the size distribution $X_{0}^{\text{old}}[r_{worst}]$.


